RoboSPA: Can VLA Models Go Beyond Simple Scenes and Short-Horizon Tasks?

Vision-Language-Action (VLA) models have shown promising progress in language-conditioned robotic manipulation. However, existing datasets and benchmarks mainly evaluate task completion under predefined settings, offering limited insight into model reasoning under increasing spatial and procedural complexity. We introduce \textbf{RoboSPA} (\textbf{Robo}t \textbf{S}patial-\textbf{P}rocedural \textbf{A}ssessment), a large-scale robotic manipulation dataset and benchmark for diagnosing embodied reasoning in VLA models. \texttt{RoboSPA} focuses on two core dimensions, Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning, covering 10 task categories and 56 base tasks. Each task is instantiated across five difficulty levels, yielding 280 variants with increasing spatial ambiguity and procedural complexity. We collect 527K trajectories across multiple embodiments and diverse scenes. Beyond binary success rate, \texttt{RoboSPA} introduces diagnostic metrics for more detailed evaluation. Experiments on representative VLA models show that current systems still struggle with complex spatial relations, precise low-level execution, and memory-intensive planning. These results establish \texttt{RoboSPA} as a challenging diagnostic benchmark for developing more capable, reliable, and generalizable embodied agents. Our data and code are available at https://github.com/fanzhenxuan/RoboSPA.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/0_abstract.tex <==
\begin{center}
    \includegraphics[width=\textwidth]{figures/benchmark.pdf}
    \captionof{figure}{\textbf{Overview} of \texttt{RoboSPA}. \texttt{RoboSPA} is built around two core dimensions: Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning, covering \textbf{10} task categories and \textbf{56} base tasks. Each base task is instantiated across \textbf{5} difficulty levels, resulting in \textbf{280} task variants. \texttt{RoboSPA} contains \textbf{527K} trajectories across multiple embodiments and scene settings. It supports step-level evaluation and is designed to diagnose VLA limitations in spatial reasoning, long-horizon execution, and complexity-scalable embodied reasoning.}    
    \label{fig:introduction}
\end{center}
\begin{abstract}
Vision-Language-Action (VLA) models have shown promising progress in language-conditioned robotic manipulation. However, existing datasets and benchmarks mainly evaluate task completion under predefined settings, offering limited insight into how models reason under increasing spatial and procedural complexity. We introduce \textbf{RoboSPA} (\textbf{Robo}t \textbf{S}patial-\textbf{P}rocedural \textbf{A}ssessment), a large-scale robotic manipulation dataset and benchmark for diagnosing embodied reasoning capabilities in VLA models. RoboSPA focuses on two core dimensions, Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning, covering 10 task categories and 56 base tasks. Each task is instantiated across five difficulty levels, resulting in 280 task variants with progressively increasing spatial ambiguity, candidate objects, action horizons, and procedural complexity. We collect 527K trajectories across multiple robotic embodiments and both clean and domain-randomized scenes. In addition to standard success rate, RoboSPA provides fine-grained metrics for spatial target grounding and long-horizon subtask completion. Experiments on representative VLA models show that current systems still struggle with complex spatial relations, order-sensitive execution, and memory-intensive planning, especially at higher difficulty levels. These results demonstrate that RoboSPA provides a challenging and diagnostic testbed for developing more robust and reasoning-aware embodied agents.
\end{abstract}

==> sections/1_introduction.tex <==
\section{Introduction}
Vision-Language-Action (VLA) models~\cite{pmlr-v229-zitkovich23a, pmlr-v270-kim25c,BlackK-RSS-25,nvidia2025gr00tn1openfoundation, intelligence2025pi05visionlanguageactionmodelopenworld} have recently emerged as a promising paradigm for building general-purpose embodied agents, enabling systems to integrate visual perception, language understanding, and action generation into a unified framework. Benefiting from large-scale pretraining and multimodal alignment~\cite{pmlr-v229-walke23a, 10611477, khazatsky2024droid}, these models demonstrate encouraging performance on language-conditioned manipulation tasks, particularly in structured environments with short-horizon interactions~\cite{li2024roboflamingo,liu2024robomamba,wen2025tinyvla}.

However, deploying embodied agents in real-world scenarios requires capabilities beyond short-horizon instruction following in simple, well-structured scenes~\cite{ma2024survey,kawaharazuka2025vision,Zhang_2025_ICCV,zhang2025vlaarena}.
Everyday manipulation tasks pose three fundamental challenges: 
(1) \textbf{Fine-grained target disambiguation}, where agents must identify the intended object among plausible candidates~\cite{garcia2025gembench,Zhang_2025_ICCV}. Real-world kitchens, desks, and dining tables often contain visually similar objects, making category- or color-based grounding insufficient;
(2) \textbf{Temporally extended task execution}, where many everyday tasks require agents to complete multiple action steps while preserving temporal constraints and handling accumulated errors~\cite{9788026,Nasiriany-RSS-24,chen2026rmbenchmemorydependentroboticmanipulation};
and (3) \textbf{Complexity-scalable embodied reasoning}, where more candidate objects, longer action horizons, and diverse environments can amplify grounding and planning failures~\cite{Pumacay-RSS-24,zhou2025liberoprorobustfairevaluation,pmlr-v270-li25c,sedlacek2025realm}. 
These challenges call for a benchmark that evaluates not only whether a VLA model can execute an action, but also whether it can reason about \textit{what} to manipulate, \textit{when} to act, and \textit{how} to maintain reliable progress under increasing complexity.

As shown in Table~\ref{tab:dataset_comparison}, existing robotic manipulation datasets and benchmarks still leave several major gaps for evaluating reasoning-oriented VLA models. 
First, fine-grained spatial reasoning is rarely evaluated explicitly, as prior works do not systematically test whether models can disambiguate targets using subtle spatial cues~\cite{garcia2025gembench,Zhang_2025_ICCV,zhang2025vlaarena}. 
In addition, long-horizon and step-level evaluation remain limited~\cite{9788026,Zhang_2025_ICCV,chen2026rmbenchmemorydependentroboticmanipulation}. 
Benchmarks such as LIBERO~\cite{liu2023libero} and RoboTwin 2.0~\cite{chen2026robotwin} mainly focus on short-horizon tasks, while long-horizon benchmarks such as RoboCasa~\cite{Nasiriany-RSS-24} and MIKASA-Robo~\cite{cherepanov2026memory} often lack step-level diagnosis of where execution fails.
Furthermore, most prior works lack controlled multi-level difficulty~\cite{Pumacay-RSS-24,fei25libero-plus,zhou2025liberoprorobustfairevaluation}, making it hard to study how performance degrades as spatial ambiguity or action horizon increases. 
Finally, dataset scale remains limited for broad reasoning evaluation. 
Although Open X-Embodiment~\cite{10611477} and recent large-scale resources~\cite{agibotworldcontributors2025agibotworldcolosseolargescale,11127809,WuK-RSS-25} expand robot data collection, many commonly used resources, such as BridgeData V2~\cite{pmlr-v229-walke23a}, contain fewer than 200K trajectories, limiting coverage across diverse tasks, embodiments, and scene settings.

To address these limitations, we introduce \textbf{RoboSPA} (\textbf{Robo}t \textbf{S}patial-\textbf{P}rocedural \textbf{A}ssessment)
, a large-scale robotic manipulation dataset and benchmark with over 500K collected trajectories. \texttt{RoboSPA} provides a unified foundation for systematically studying embodied reasoning under increasing task complexity, moving beyond standard task completion toward more diagnostic evaluation of VLA model capabilities.
These goals motivate three core design principles: Fine-Grained Spatial Reasoning, Long-Horizon Procedural Planning, and Multi-Level Hierarchical Evaluation.

\begin{itemize}[leftmargin=12pt]
\item \textbf{Fine-Grained Spatial Reasoning:} 
As shown in Fig.~\ref{fig:introduction}, this component evaluates whether VLA models can ground language instructions in complex spatial structures across five categories: geometric attribute cognition, spatial distance estimation, cross-view reasoning, referential relational understanding, and canonical position indexing. This capability is essential for robotic manipulation, since robots often need to distinguish subtle spatial cues and select the correct target from cluttered scenes. To the best of our knowledge, \texttt{RoboSPA} is the first VLA dataset to systematically focus on fine-grained spatial reasoning as a core evaluation dimension.
\input{tables/datasets}
\item \textbf{Long-Horizon Procedural Planning:} 
This component evaluates whether VLA models can execute temporally extended manipulation tasks that require sustained decision making over multiple steps. As shown in Fig.~\ref{fig:introduction}, it consists of five categories: repetitive procedure following, order-constrained execution, order-free execution, Composite Action Coordination, and memory-intensive planning. While the first four categories evaluate common long-horizon procedural patterns, memory-intensive planning further tests whether agents can retain and use intermediate task states over extended horizons. This capability is essential for robotic manipulation, since real-world tasks often require temporal consistency and reliable progress across multiple steps.
\item \textbf{Multi-Level Hierarchical Evaluation:} The multi-level hierarchical evaluation component measures how VLA model performance changes under progressively increasing task complexity. Each base task is instantiated across five difficulty levels, enabling systematic analysis of performance degradation as spatial complexity and action horizons grow. In addition to task-level success, \texttt{RoboSPA} further reports step-level progress, providing a more fine-grained diagnosis of model failures beyond binary success or failure.
\end{itemize}

Overall, \texttt{RoboSPA} is constructed as a large-scale VLA dataset with carefully controlled task design and trajectory collection. 
All trajectories are collected using manually designed expert code, which is strictly inspected to ensure correct task logic and reliable execution. 
For each task, we collect demonstrations under both clean and domain-randomized scenes, enabling evaluation in controlled settings as well as visually and spatially diverse environments. 
In total, \texttt{RoboSPA} contains 56 base tasks across 10 capability categories, with each task instantiated at five difficulty levels, resulting in 280 task variants. 
This hierarchical task design further supports step-level diagnostic evaluation, allowing models to be assessed beyond final success rates. 
Using five robotic embodiments, we collect 527K trajectories in total, corresponding to 997 hours of interaction videos and 108M timesteps.
Together, these properties provide a large-scale dataset for evaluating embodied reasoning under increasing spatial and procedural complexity.

We evaluate representative VLA models~\cite{Brohan-RSS-23, agibotworldcontributors2025agibotworldcolosseolargescale, intelligence2025pi05visionlanguageactionmodelopenworld, zheng2026xvla} on \texttt{RoboSPA} and find that existing models still struggle under increasing spatial and procedural complexity. 
In particular, the success rates of all evaluated models remain below 25\% on the most difficult tasks, with some tasks even receiving 0\% success, revealing substantial limitations in current VLA systems.
Through diagnostic analyses, we further identify representative failure modes and show that future VLA models should strengthen fine-grained target grounding, precise low-level execution, long-horizon progress tracking, and memory-based reasoning. 
These findings suggest that \texttt{RoboSPA} serves not only as a challenging benchmark, but also as a diagnostic testbed for guiding future progress in embodied reasoning.

==> sections/2_related_work.tex <==

\section{Related Work}
\label{sec:related_work}

\paragraph{Vision-Language-Action Models.}
Vision-Language-Action (VLA) models integrate visual perception, language understanding, and robot control by generating robot actions conditioned on visual observations and language instructions. Early embodied multimodal systems, including RT-2~\citep{pmlr-v229-zitkovich23a}, PaLM-E~\citep{10.5555/3618408.3618748}, and VIMA~\citep{pmlr-v202-jiang23b}, showed that semantic knowledge from large-scale vision-language data can improve robotic instruction following and object grounding. OpenVLA~\citep{pmlr-v270-kim25c} and Octo~\citep{ghosh2024octo} further advanced open-source and generalist robot policies. However, autoregressive action-token VLAs can be computationally expensive and may be less suitable for high-frequency continuous control. Recent work improves action generation through flow-matching action heads, diffusion-based policies, compact deployment, and cross-embodiment scaling, as shown by the $\pi$~family~\citep{BlackK-RSS-25,intelligence2025pi05visionlanguageactionmodelopenworld}, RDT~\citep{liu2025rdtb}, SmolVLA~\citep{shukor2025smolvla}, and X-VLA~\citep{zheng2026xvla}. Other efforts explore hierarchical or latent actions, temporal memory, spatial guidance, multi-frame context, and parameter-efficient adaptation~\citep{Belkhale-RSS-24,BuQ-RSS-25,ICLR2025_8667f264,zhang2025dreamvla,shi2026memoryvla,liu2026ttfvla,chen2025internvlam1spatiallyguidedvisionlanguageaction,jang2025contextvlavisionlanguageactionmodelamortized,wang2025vlaadaptereffectiveparadigmtinyscale}. These advances make VLA policies more practical, but their evaluations often conflate perception, spatial grounding, temporal state tracking, and procedural planning errors, making it difficult to diagnose failures in spatial and long-horizon reasoning.

\paragraph{Robotic Manipulation Datasets and Benchmarks.}
Robot manipulation datasets and benchmarks have evolved alongside robotic policies. Early simulated benchmarks such as RLBench~\citep{james2020rlbench}, ManiSkill2~\citep{gumaniskill2}, and CALVIN~\citep{9788026} standardize diverse manipulation skills, with RLBench and CALVIN further supporting language-conditioned and long-horizon evaluation. LIBERO~\citep{liu2023libero} studies transfer and compositional generalization. In parallel, large-scale datasets such as BridgeData V2~\citep{pmlr-v229-walke23a}, Open X-Embodiment~\citep{10611477}, DROID~\citep{khazatsky2024droid}, DexMimicGen~\citep{11127809}, AgiBot World/Colosseo~\citep{agibotworldcontributors2025agibotworldcolosseolargescale}, and DexUMI~\citep{WuK-RSS-25} expand real-world, cross-embodiment, and dexterous manipulation coverage. Recent benchmarks target more specific generalization failures: The Colosseum~\citep{Pumacay-RSS-24} studies perturbation robustness; RoboCasa~\citep{Nasiriany-RSS-24} scales household scenes; SimplerEnv~\citep{pmlr-v270-li25c} and REALM~\citep{sedlacek2025realm} study sim-to-real transfer; GemBench~\citep{garcia2025gembench} and VLABench~\citep{Zhang_2025_ICCV} add placement, language, object, and long-horizon variations; LIBERO-Plus~\citep{fei25libero-plus}, LIBERO-Pro~\citep{zhou2025liberoprorobustfairevaluation}, VLA-Arena~\citep{zhang2025vlaarena}, RoboTwin 2.0~\citep{chen2026robotwin}, and RMBench~\citep{chen2026rmbenchmemorydependentroboticmanipulation} further study robustness, difficulty factors, bimanual data generation, and memory-dependent manipulation. Despite broader evaluation coverage, existing benchmarks rarely isolate fine-grained spatial reasoning and long-horizon procedural planning with step-level diagnostics. Our benchmark fills this gap with RoboTwin-based tasks organized along these two axes, reporting both difficulty-level success and step-level progress to localize failures beyond binary final success.



==> sections/3_benchmark.tex <==
\section{RoboSPA}
\label{headings}
\subsection{Overview}
As shown in Fig.~\ref{fig:overview}, we introduce \texttt{RoboSPA}, a large-scale robotic manipulation dataset and benchmark for evaluating VLA models beyond short-horizon imitation, focusing on two core capabilities: Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning. The benchmark consists of 56 tasks in total and is developed using the SAPIEN~\cite{9156706} simulator and the RoboTwin 2.0~\cite{chen2026robotwin} framework. Each task is further instantiated across multiple difficulty levels, enabling controlled evaluation of model performance under increasing spatial complexity and procedural length. The former tests whether models can understand subtle object attributes, spatial relations, viewpoints, and positional structures, while the latter evaluates multi-step behaviors requiring repetition, ordering, memory, and compositional execution. Overall, the benchmark provides a structured and diagnostic evaluation of embodied reasoning, revealing limitations that are often hidden by coarse success-rate metrics.

\begin{figure*}[t]
\centering
\begin{minipage}{0.43\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/category.pdf}
    {\footnotesize \caption*{(a) Capability taxonomy}}
\end{minipage}
\hfill
\begin{minipage}{0.55\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/1.pdf}
    {\footnotesize \caption*{(b) Multi-difficulty task design}}
    
    \vspace{0.8em}
    
    \includegraphics[width=\linewidth]{figures/randomized.png}
    {\footnotesize \caption*{(c) Domain-randomized scenes}}
\end{minipage}

\caption{
(a) Dataset taxonomy with two capability dimensions and 10 task categories. 
(b) Multi-difficulty design: fine-grained spatial tasks get harder with more objects, long-horizon procedural tasks with longer action sequences. 
(c) Domain-randomized scene examples with variations in object layout, distractors, lighting, textures, and tabletop configurations.
}
\label{fig:overview}
\end{figure*}

\subsection{Benchmark Construction}
\subsubsection{Capability Taxonomy}

To systematically evaluate embodied reasoning in VLA models, we construct a hierarchical capability taxonomy rather than treating manipulation tasks as isolated instances. As shown in Fig.~\ref{fig:overview}(a), the taxonomy is organized around two core dimensions: Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning, each further divided into five fine-grained capability categories. This design enables interpretable analysis of model failures across different reasoning requirements.

\paragraph{Fine-Grained Spatial Reasoning.}
This dimension assesses a model's ability to ground language instructions in detailed spatial structures. In this dimension, all tasks are formulated as pick-based manipulation, where the model must identify and pick the correct target object from a scene. Compared with simple object-centric manipulation, these tasks require models to select targets through fine-grained spatial reasoning under increasingly complex scenes. We divide this dimension into five categories:

\begin{itemize}[leftmargin=*, itemsep=0.3em]
    \item \textbf{Geometric Attribute Cognition (GAC):} Evaluates whether the model can identify and manipulate objects based on geometric or shape-related attributes. These tasks require the model to perceive object forms beyond category-level recognition and use such attributes for target selection.

    \item \textbf{Spatial Distance Estimation (SDE):} Measures the model's ability to compare distances among objects or between an object and a reference entity. The model must reason about proximity, remoteness, and relative distance rather than relying only on appearance cues.

    \item \textbf{Canonical Position Indexing (CPI):} Evaluates whether the model can identify objects by row-column indexed positions, such as a specified row and column. These tasks vary the counting direction, requiring the model to interpret indices under different spatial scanning orders.

    \item \textbf{Referential Relational Understanding (RRU):} Assesses the model's ability to locate a target object through directional spatial relations to reference objects, such as left of, in front of, and front-left of. These tasks require the model to reason over basic and compositional relative positions.
    
    \item \textbf{Cross-View Reasoning (CVR):} Examines whether the model can interpret spatial instructions from viewpoints different from the robot's egocentric observation. These tasks test the ability to transform spatial references across perspectives, such as left-view or right-view descriptions.
\end{itemize}

\paragraph{Long-Horizon Procedural Planning.}
This dimension evaluates a model's ability to complete temporally extended manipulation tasks that involve diverse action primitives, multiple subgoals, intermediate states, and procedural constraints. Unlike short-horizon tasks, these tasks require the model to track progress, preserve action consistency, and avoid errors accumulating over time. We divide this dimension into five categories:

\begin{itemize}[leftmargin=*, itemsep=0.3em]
    \item \textbf{Repetitive Procedure Following (RPF):} Assesses whether the model can repeat a specified operation for the required number of times. The model must track repetition progress and stop after completing the required iterations.
    
    \item \textbf{Order-Free Execution (OFE):} Measures whether the model can complete multiple required subgoals when the execution order is flexible. The key challenge is to cover all required targets without omission or unnecessary repetition.
    
    \item \textbf{Order-Constrained Execution (OCE):} Evaluates whether the model can execute a sequence of subgoals in a specified order. These tasks require strict temporal compliance, where completing the correct actions in the wrong order may still lead to failure.

    \item \textbf{Composite Action Coordination (CAC):} Examines the model's ability to combine heterogeneous manipulation skills into a coherent procedure. These tasks often involve multiple stages with different action types, requiring coordination across subtasks.

    \item \textbf{Memory-Intensive Planning (MIP):} Tests whether the model can use previously observed information to guide later actions, especially when relevant objects, states, or spatial configurations are no longer visible. These tasks evaluate temporal memory and state tracking during execution.
\end{itemize}

Overall, this taxonomy provides a structured diagnostic framework for VLA evaluation. The spatial dimension reveals failures in object grounding, distance comparison, perspective transformation, relational understanding, and spatial indexing. The long-horizon dimension exposes failures in ordering, subgoal coverage, behavior composition, repeated execution, and memory-based planning.

\subsubsection{Task Suite Construction}

\paragraph{Task Construction.}
Based on the proposed capability taxonomy, we design each task to instantiate a specific reasoning requirement rather than merely varying object categories or visual appearances. Each task is defined by expert code, which specifies the scene layout, action execution procedure, and success condition. 
We design the execution procedures to match the intended reasoning capability, while reusing some action primitives from RoboTwin 2.0~\cite{chen2026robotwin} when applicable.
To ensure the correctness of task construction, ten highly trained graduate students participate in the design process, with each student responsible for one capability category. After the initial design, each task is checked by two additional students to verify whether the scene setup, execution logic, and success checker are consistent with the intended reasoning capability. This cross-checking process reduces ambiguous task definitions and ensures that model failures can be attributed to the targeted capability.

\paragraph{Hierarchical Difficulty Design.}
To provide fine-grained evaluation, we instantiate each task with five difficulty levels rather than a single setting. 
As shown in Fig.~\ref{fig:overview}(b), we define difficulty levels according to the structure of each task type. 
For fine-grained spatial reasoning tasks, higher levels increase the number of candidate objects; for long-horizon procedural planning tasks, higher levels extend the action sequence with more intermediate steps.
This protocol allows us to analyze how model performance changes as the reasoning burden increases.
\paragraph{Instruction Design.}
For each task, we use GPT-5.4~\cite{singh2025openaigpt5card} to generate 60 non-overlapping instruction templates with diverse linguistic forms, where 50 are used for training and 10 for testing. These templates are further instantiated with task-specific object descriptions, such as object categories, colors, to produce diverse natural language instructions. All templates are manually checked for semantic correctness, clarity, executability, and consistency with the task specification. This design increases linguistic diversity while preserving controlled task semantics.

\subsubsection{Data Collection}
After completing the task design, we execute the expert code in the simulator to collect expert trajectories.

For each task variant, we collect trajectories under both clean and domain-randomized scene settings. Clean scenes contain only task-relevant objects, while domain-randomized scenes, as illustrated in Fig.~\ref{fig:overview}(c), introduce variations in object clutter, background textures, lighting conditions, and tabletop configurations. These two settings allow us to evaluate both basic task competence in controlled environments and robustness under more visually diverse and realistic scenes.

To capture diverse execution patterns across different kinematics and support embodiment-aware evaluation, we collect data using five robotic embodiments, including Aloha-AgileX, ARX-X5, Piper, Franka, and UR5.
For each robotic embodiment, we aim to collect 50 trajectories under clean scenes and 500 trajectories under domain-randomized scenes for every task variant. 
Due to task difficulty, embodiment-specific kinematic constraints, and motion-planning failures, some embodiment-task pairs fall short of this target. Under a limited computational budget, we retain the successfully collected trajectories rather than exhaustively resampling failed cases.

\subsubsection{Evaluation Metrics}
We use \textit{Success Rate} ($\mathcal{SR}$) as the primary metric for our benchmark, where a rollout is considered successful only if the final task-specific condition is satisfied. 

To provide more diagnostic evaluation, we further introduce two dimension-specific complementary metrics.

For fine-grained spatial reasoning tasks, different scenes may contain different numbers of candidate objects, making raw target accuracy biased by the random-guessing probability. 

To fairly compare spatial reasoning ability under varying scene complexity, we introduce \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$), inspired by Cohen's kappa~\citep{cohen1960coefficient}, which adjusts observed agreement by its chance-level expectation.
$\mathcal{ONTA}$ removes the object-count-induced chance baseline:
\begin{equation}
\mathcal{ONTA}(n)
=
\left(
\frac{\mathcal{SR}(n)-1/n}{1-1/n}
\right)
\times 100 .
\label{eq:onta}
\end{equation}
where \(n\) is the number of candidate objects. 
$\mathcal{ONTA}$ reaches 100 when all targets are correctly selected, 0 at random-guessing performance, and can be negative when performance falls below chance.

For long-horizon procedural planning tasks, we report \textit{Progress Score} ($\mathcal{PS}$) to capture partial completion beyond binary success. 
It is computed on a 0--100 scale:
\begin{equation}
\mathcal{PS}
=
\left(
\frac{1}{N}\sum_{i=1}^{N}\frac{c_i}{T}
\right)
\times 100 .
\label{eq:progress}
\end{equation}
where \(T\) denotes the total number of subtasks for the task, and \(c_i\) denotes the number of completed subtasks in episode \(i\).

\begin{figure*}[t]
    \centering

    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stat_1.pdf}
        \caption{Embodiment Distribution}
        \label{fig:stat_a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stat_2.pdf}
        \caption{Scene Distribution}
        \label{fig:stat_b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stat_3.pdf}
        \caption{Average timesteps}
        \label{fig:stat_c}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stat_4.pdf}
        \caption{Average object count}
        \label{fig:stat_d}
    \end{subfigure}

    \caption{\textbf{Dataset statistics} of \texttt{RoboSPA}. 
    (a) Trajectory distribution across five robotic embodiments. 
    (b) Trajectory distribution between clean and domain-randomized scenes. 
    (c) Average trajectory length, measured by timesteps, across difficulty levels for long-horizon procedural planning tasks. 
    (d) Average number of objects across difficulty levels for fine-grained spatial reasoning tasks.}
    \label{fig:statistics}
\end{figure*}

\subsection{Benchmark Statistics}
\texttt{RoboSPA} contains \textbf{56} base tasks across two capability dimensions, including \textbf{24} tasks for Fine-Grained Spatial Reasoning and \textbf{32} tasks for Long-Horizon Procedural Planning. 
Each dimension is further divided into five task categories, resulting in 10 task categories in total. 
Each base task is instantiated at 5 difficulty levels, yielding \textbf{280} task variants. 
In total, we collect approximately \textbf{527K} trajectories, corresponding to over \textbf{997} hours of interaction videos and \textbf{108M} timesteps.

The environments contain 581 distinct objects from 120 object categories across daily manipulation scenarios, with substantial variation in geometry, appearance, and spatial configuration. 
To support language-conditioned evaluation, we design 5280 instruction templates with diverse linguistic forms. 
The collected trajectories span \textbf{5} robotic embodiments, with the embodiment distribution shown in Fig.~\ref{fig:statistics}(a). 
As shown in Fig.~\ref{fig:statistics}(b), the dataset contains 64K trajectories from clean scenes and 463K trajectories from domain-randomized scenes. 
Fig.~\ref{fig:statistics}(c) and Fig.~\ref{fig:statistics}(d) further illustrate the hierarchical difficulty design: higher-level fine-grained spatial reasoning tasks involve more candidate objects, while higher-level long-horizon procedural planning tasks require more timesteps.

==> sections/4_experiment.tex <==

\section{Experiments}
\label{others}

\subsection{Experimental Setup}
We evaluate four representative VLA models: RDT~\cite{liu2025rdtb}, $\pi_{0.5}$~\cite{intelligence2025pi05visionlanguageactionmodelopenworld}, GO-1~\cite{agibotworldcontributors2025agibotworldcolosseolargescale}, and X-VLA~\cite{zheng2026xvla}. For a controlled comparison, we use the clean-scene data collected with the Aloha-AgileX embodiment for both training and evaluation. 
All models are trained and evaluated under a single-task setting. For each base task, we train a separate model using data from all five difficulty levels and evaluate it independently at each level.
During evaluation, each model is tested with 100 rollout trials per task variant. We report \textit{Success Rate} ($\mathcal{SR}$) for all tasks, \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$) for Fine-Grained Spatial Reasoning tasks, and \textit{Progress Score} ($\mathcal{PS}$) for Long-Horizon Procedural Planning tasks.

\subsection{Main Results}
\input{tables/main_table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/category_lines/category_success_rates_10panels.pdf}
    \caption{
    Success rate trends of four baseline VLA models across 10 task categories over five difficulty levels}
    \label{fig:category_success_rates}
\end{figure*}



Table~\ref{tab:main_results} presents the main comparison across four representative VLA models. Overall, all models exhibit a clear performance decline from L1 to L5, with the overall \textit{Success Rate} drop ranging from 9.9\% to 32.9\% across models. 
This shows that success on simple instances does not reliably transfer to harder spatial configurations or longer procedural horizons.

% \paragraph{Model Comparison.}
% Among the evaluated models, $\pi_{0.5}$ achieves the best overall performance, followed by X-VLA. However, both models still suffer substantial degradation as difficulty increases, with drops of 33.0 and 30.7 percentage points, respectively. This suggests that stronger models perform better on easy cases, but still lack robust reasoning ability under more complex conditions.


\paragraph{Model Comparison.}
Among the evaluated models, $\pi_{0.5}$ achieves the best overall performance, but reaches only 22.3\% success rate at L5, followed by X-VLA with only 19.9\% at L5. 
Moreover, both models still suffer substantial degradation as difficulty increases, with drops exceeding 30 percentage points.
GO-1 and RDT perform worse overall, achieving only 8.8\% and 6.9\% success rates at L5, respectively.
These results suggest that stronger models perform better on easier cases, but all models still lack robust reasoning ability under more complex conditions.

% \paragraph{Fine-Grained Spatial Reasoning.}
% In this dimension, X-VLA achieves the strongest average performance. Models struggle particularly with relational grounding and spatial indexing, where the hardest-level average performance remains low. This indicates that current VLA models are still unreliable when target selection depends on fine-grained spatial relations rather than simple object recognition.

\paragraph{Fine-Grained Spatial Reasoning.}
X-VLA shows the best performance in this dimension, but its success rate still drops from 41.9\% at L1 to only 23.9\% at L5. This decline shows that increasing spatial complexity substantially weakens target grounding. 
Models struggle particularly with Canonical Position Indexing (CPI) and Referential Relational Understanding (RRU), indicating that current VLA models remain unreliable when target selection depends on fine-grained spatial relations rather than simple object recognition.

\paragraph{Long-Horizon Procedural Planning.}
For Long-Horizon Procedural Planning, the degradation is more severe, with model-wise \textit{Success Rate} decreases ranging from 16.4\% to 48.1\% from the most difficult to the easiest tasks. 
Models perform best on Repetitive Procedure Following (RPF), while the other four categories show substantially lower performance.
Notably, all models fail on the hardest Memory-Intensive Planning (MIP), revealing severe limitations in maintaining task-relevant memory over extended horizons.

Overall, these results demonstrate the diagnostic value of our benchmark. The multi-level design not only measures task success, but also reveals how model capabilities degrade as spatial and procedural reasoning demands increase.
Fig.~\ref{fig:benchmark_radar} visualizes model performance across ten capability categories under the easiest and hardest settings. 
On L1, stronger models cover more categories but still show uneven performance, especially on fine-grained spatial reasoning tasks. 
On L5, performance drops sharply across most task categories, exposing failures in both spatial discrimination and long-horizon procedural tracking, consistent with Table~\ref{tab:main_results}.

\input{tables/table2}
\input{tables/table3}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/benchmark_radar.png}
%     \caption{Comparison of mainstream VLA models on \texttt{RoboSPA}. \textbf{Left}}: Performance on   ten evaluation categories under the easiest task setting (L1). \textbf{Right}: Performance on the same categories under the hardest task setting (L5).}
% \label{fig:benchmark_radar}
% \end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/benchmark_radar.png}
    \caption{
    Comparison of four baseline VLA models on \texttt{RoboSPA}.
    \textbf{Left:} \textit{Success Rate} trends of four baseline models across 10 task categories under the easiest task setting (L1). 
    \textbf{Right:} Performance under the hardest task setting (L5) on the same categories.
    }
    \label{fig:benchmark_radar}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fail_example.pdf}
    \caption{
    Representative failure modes observed in our diagnostic analysis. 
    % The six illustrated errors are: 
    % \textbf{① Target Execution Error}, 
    % \textbf{② Target Grounding Error}, 
    % \textbf{③ Manipulation Error}, 
    % \textbf{④ Memory Error}, 
    % \textbf{⑤ Temporal Ordering Error}, and 
    % \textbf{⑥ Redundant Repetition Error}. 
    % These cases highlight limitations in spatial reasoning, low-level manipulation, long-horizon planning, and memory-based reasoning.
    }
    \label{fig:fail_example}
\end{figure*}

\subsection{Fine-Grained Evaluation Beyond Binary Success}

\paragraph{Object-Normalized Target Accuracy.}
To better reflect models' true target-grounding ability in fine-grained spatial reasoning tasks, Table~\ref{tab:onta_spatial} compares models using the $\mathcal{ONTA}$ metric.
Overall, $\mathcal{ONTA}$ remains low across models, indicating that many spatial failures arise from incorrect target grounding rather than manipulation errors alone. 
RDT and GO-1 obtain negative $\mathcal{ONTA}$ on almost all categories and difficulty levels, suggesting that they exhibit little reliable spatial reasoning ability beyond random selection. 
$\pi_{0.5}$ and X-VLA show fewer negative scores and achieve better average $\mathcal{ONTA}$, but their overall scores remain close to the random-selection baseline. 
These results suggest that current VLA models still struggle to identify the correct target when success depends on fine-grained attributes, spatial relations, viewpoints, or ordinal positions.

\paragraph{Long-Horizon Subtask Completion.}
Table~\ref{tab:long_horizon_completion} reports \textit{Progress Score} for long-horizon procedural planning tasks, providing a progress-based view beyond binary \textit{Success Rate}.
The results show that \textit{Progress Score} is generally higher than final \textit{Success Rate}, indicating that models can often execute part of a procedure but fail due to accumulated errors, incorrect ordering, or incomplete later-stage execution. $\pi_{0.5}$ achieves the strongest average completion rate, followed by X-VLA. 
Nevertheless, Memory-Intensive Planning (MIP) remains weak at higher difficulty levels, indicating that current models still have limited memory ability during long-horizon execution.


% \subsection{Analysis}
\subsection{Qualitative Results}
Fig.~\ref{fig:benchmark_radar} visualizes category-wise model performance across task difficulty. 
The radar plots show that model performance is highly uneven across categories and shrinks markedly under harder settings. 
This highlights persistent weaknesses in fine-grained spatial grounding, ordered execution, and memory-dependent planning.

\subsection{Diagnostic Analysis}

To better understand the limitations of current VLA models, we conduct a comprehensive error analysis on the two best-performing models, $\pi_{0.5}$ and X-VLA. 
Detailed quantitative breakdowns are provided in the Appendix. 
Based on the analyzed failed rollouts, we summarize the major failure modes into six representative error categories, as illustrated in Fig.~\ref{fig:fail_example}.

\paragraph{Error Analysis.}
For fine-grained spatial reasoning, we observe two major errors. 
Target execution error occurs when the model identifies the correct target but fails to manipulate it successfully, revealing a gap between visual grounding and physical execution. 
Target grounding error occurs when the model selects an incorrect object among distractors, indicating insufficient fine-grained spatial discrimination.

For long-horizon procedural planning, failures are more diverse. 
Manipulation error refers to inaccurate execution of an intermediate action, which may block subsequent steps. 
State memory error occurs when the model fails to retain task-relevant information observed earlier. 
Temporal ordering error indicates that valid subtasks are executed in the wrong sequence. 
Redundant repetition error occurs when the model repeats an already completed action instead of progressing to the next subgoal.

\paragraph{Implications for Future Models.}
% These diagnostic results suggest several directions for future VLA models. 
% To improve spatial reasoning, future policies should strengthen object-centric and relation-aware grounding to distinguish targets from distractors under complex layouts. 
% Beyond accurate grounding, long-horizon tasks require explicit progress tracking, enabling models to recognize completed subtasks and avoid ordering mistakes or unnecessary repetitions. 
% In addition, memory mechanisms are needed for scenarios where correct decisions depend on earlier observations or hidden states. 
% Finally, execution monitoring and recovery are important for preventing local manipulation failures from cascading into complete task failure.

These diagnostic results suggest several directions for future VLA models. 
To improve spatial reasoning, future policies should strengthen object-centric and relation-aware grounding to distinguish targets from distractors under complex layouts. 
In addition, precise low-level execution is critical for all tasks, ensuring that actions such as grasping, pressing, or moving are carried out reliably.
Beyond grounding and execution, long-horizon tasks require explicit progress tracking, enabling models to recognize completed subtasks and avoid ordering mistakes or unnecessary repetitions. 
Memory mechanisms are needed for scenarios where correct decisions depend on earlier observations or hidden states. 
Finally, execution monitoring and recovery are important for preventing local manipulation failures from cascading into complete task failure.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/benchmark_radar.png}
%     \caption{Comparison of mainstream VLA models on \texttt{RoboSPA}. Left: Performance on   ten evaluation categories under the easiest task setting (L1). Right: Performance on the same categories under the hardest task setting (L5).}
% \label{fig:benchmark_radar}
% \end{figure*}





==> sections/5_conclusion.tex <==

\section{Conclusion}
In this paper, we present \texttt{RoboSPA}, a large-scale robotic manipulation dataset and benchmark for evaluating reasoning-oriented Vision-Language-Action models. Built around Fine-Grained Spatial Reasoning and Long-Horizon Procedural Planning, \texttt{RoboSPA} covers ten task categories and instantiates each base task across five difficulty levels, enabling systematic analysis of how model performance changes with increasing task complexity. We further provide trajectories across multiple embodiments and both clean and domain-randomized scenes, together with fine-grained metrics for spatial grounding and subtask completion. Experiments on representative VLA models show that current models still struggle with complex spatial relations, order-sensitive execution, and memory-intensive planning, especially at higher difficulty levels. We hope this benchmark can serve as a diagnostic testbed for developing more robust and reasoning-aware embodied agents.

==> tables/all_tasks.tex <==
\begin{table}[H]
\centering
\caption{Task list and descriptions for fine-grained spatial reasoning. Category abbreviations: GAC = Geometric Attribute Cognition, SDE = Spatial Distance Estimation, CVR = Cross-View Reasoning, CPI = Canonical Position Indexing, and RRR = Referential Relational Reasoning.}
\label{tab:spatial_task_list}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\textwidth}{p{0.07\textwidth} p{0.30\textwidth} X}
\toprule
\textbf{Cat.} & \textbf{Task Name} & \textbf{Task Description} \\
\midrule
GAC & Pick Blocks Size & Pick the target block from multiple blocks based on the size. \\
GAC & Pick Blocks Height & Pick the target block from multiple blocks based on the height. \\
GAC & Pick Blocks Length & Pick the target block from multiple blocks based on the length. \\
GAC & Pick Blocks Area & Pick the target block from multiple blocks based on the base area. \\

SDE & Pick Blocks Distance & Pick the target block from multiple blocks using both color and relative distance cues. \\
SDE & Pick Mugs Distance & Pick the target mug from multiple mugs using both color and relative distance cues. \\
SDE & Pick Pill Bottles Distance & Pick the target pill bottle from multiple pill bottles using both color and relative distance cues. \\
SDE & Pick Mixed Objects Distance A & Pick the target object from mixed-object set A using both color and relative distance cues. \\
SDE & Pick Mixed Objects Distance B & Pick the target object from mixed-object set B using both color and relative distance cues. \\

CPI & Pick Blocks Canonical & Pick the target block according to its ordinal position among multiple blocks. \\
CPI & Pick Cups Canonical & Pick the target cup according to its ordinal position among multiple cups. \\
CPI & Pick Rubik Cubes Canonical & Pick the target Rubik cube according to its ordinal position among multiple Rubik cubes. \\
CPI & Pick Mixed Objects Canonical A & Pick the target object from mixed-object set A according to ordinal position. \\
CPI & Pick Mixed Objects Canonical B & Pick the target object from mixed-object set B according to ordinal position. \\

RRR & Pick Tea Box Relational & Pick the target tea box according to its relative position to another reference tea box. \\
RRR & Pick Cans Relational & Pick the target can according to its relative position to another reference can. \\
RRR & Pick Soaps Relational & Pick the target soap according to its relative position to another reference soap. \\
RRR & Pick Mixed Objects Relational A & Pick the target object in a mixed-object scene according to another reference object. \\
RRR & Pick Mixed Objects Relational B & Pick the target object in a mixed-object scene according to another reference object. \\

CVR & Pick Sauce Can Multi View & Pick up the target sauce can specified by its absolute position under a given viewpoint. \\
CVR & Pick Seals Multi View & Pick up the target seal specified by its absolute position under a given viewpoint. \\
CVR & Pick Breads Multi View & Pick up the target bread specified by its absolute position under a given viewpoint. \\
CVR & Pick Mixed Objects Multi View A & Pick up the target object from mixed-object group A specified by its absolute position under a given viewpoint. \\
CVR & Pick Mixed Objects Multi View B & Pick up the target object from mixed-object group B specified by its absolute position under a given viewpoint. \\

\bottomrule
\end{tabularx}
\end{table}

% \bottomrule
% \end{tabularx}
% \end{center}

\begin{table}[H]
\centering
\caption{Task list and descriptions for long-horizon procedural planning. Category abbreviations: RPF = Repetitive Procedure Following, OFE = Order-Free Execution, OCE = Order-Constrained Execution, CAC = Composite Action Coordination, and MIP = Memory-Intensive Planning.}
\label{tab:long_horizon_task_list}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\textwidth}{p{0.07\textwidth} p{0.30\textwidth} X}
\toprule
\textbf{Cat.} & \textbf{Task Name} & \textbf{Task Description} \\
\midrule

RPF & Press Stapler Repeat & Press the stapler repeatedly. \\
RPF & Lift Pot Repeat & Lift and put down the pot repeatedly. \\
RPF & Lift Fan Repeat & Lift the fan repeatedly. \\
RPF & Click Bell Repeat & Click the bell repeatedly. \\

OFE & Put Bottles Dustbin & Put multiple bottles into the dustbin without requiring a fixed execution order. \\
OFE & Move Blocks Apart & Move multiple blocks apart without requiring a fixed execution order. \\
OFE & Move Playing Cards Away & Move multiple playing cards away without requiring a fixed execution order. \\
OFE & Place Bowls Plates & Place multiple bowls on plates without requiring a fixed execution order. \\
OFE & Separate Fries Bread & Separate fries and bread into different areas without requiring a fixed execution order. \\
OFE & Rank Blocks Height & Arrange multiple blocks by height while allowing flexible intermediate execution order. \\
OFE & Rank Blocks Color & Arrange multiple blocks by color while allowing flexible intermediate execution order. \\
OFE & Rank Blocks Size & Arrange multiple blocks by size while allowing flexible intermediate execution order. \\

OCE & Hit Blocks Hammer Order & Hit multiple blocks with a hammer in the specified color order. \\
OCE & Click Objects Order & Click multiple target objects in the specified order. \\
OCE & Stamp Seals Order & Stamp multiple seals in the specified order. \\
OCE & Click Bell Clockwise Order & Click the bell and then execute the clockwise movement sequence in order. \\
OCE & Stack Blocks Color Order & Stack multiple blocks in the specified color order. \\
OCE & Stack Blocks Size Order & Stack multiple blocks in the specified size order. \\
OCE & Stack Blocks Length Order & Stack multiple blocks in the specified length order. \\

CAC & Place Phone Press Stapler & Execute a manipulation task involving phone placement, repeated pressing, and dumping. \\
CAC & Place Bottle Cup & Execute a manipulation task involving throwing bottles into a dustbin and placing cups on coasters. \\
CAC & Hang Mug Stack Blocks & Execute a manipulation task involving hanging a mug on a rack and stacking blocks from bottom to top. \\
CAC & Place Object Scale Click & Execute a manipulation task involving object placement, pressing, and returning objects to the table. \\
CAC & Place Burger Fries Click Bell & Execute a manipulation task involving placing a hamburger and fries on a tray, clicking a bell, and returning them. \\
CAC & Click Can Place Items & Execute a manipulation task involving interleaved can clicking with placing bread in a basket and a pill bottle on a pad. \\
CAC & Stamp Seals Press Stapler & Execute a manipulation task involving stamping left and right seals twice on their pads and pressing a stapler. \\
CAC & Click Bell Open Microwave Place Object & Execute a manipulation task involving interleaved bell clicking, opening a microwave, and placing an object left of another. \\

MIP & Observe Blocks Move Memory & First remember the colors of the display blocks, then move matching blocks on the table closer after the display blocks are hidden. \\
MIP & Observe Objects Click Memory & First remember the objects on the display platform from left to right, then click matching objects on the table in the same order after they are hidden. \\
MIP & Remember Color Cover & First remember the block colors, then uncover the blocks in the given color order after they are covered. \\
MIP & Remember Orientation Restore & First remember the orientations of the front T-shaped blocks, then adjust the rear T-shaped blocks to match them from left to right after they are hidden. \\
MIP & Press Stapler Memory & Remember how many times each stapler should be pressed and then press them. \\

\bottomrule
\end{tabularx}
\end{table}

==> tables/assets.tex <==
\begin{table}[H]
\centering
\caption{Asset categories and the number of variants used in RoboSPA.}
\label{tab:asset_categories}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lclclclc}
\toprule
\textbf{Asset} & \textbf{\#Var.} &
\textbf{Asset} & \textbf{\#Var.} &
\textbf{Asset} & \textbf{\#Var.} &
\textbf{Asset} & \textbf{\#Var.} \\
\midrule
bottle & 27 & olive-oil & 5 & pencup & 7 & globe & 2 \\
bowl & 7 & drill & 7 & kitchenpot & 7 & trophy & 5 \\
cover & 1 & jam-jar & 5 & battery & 6 & notebook & 3 \\
plate & 1 & screwdriver & 1 & plasticbox & 11 & brush-pen & 6 \\
fluted-block & 2 & fork & 1 & tabletrashbin & 11 & rest & 4 \\
french-fries & 4 & knife & 1 & msg & 6 & glue & 6 \\
hamburg & 6 & apple & 2 & soy-sauce & 5 & cleaner & 4 \\
T\_block & 2 & cabinet & 1 & vinegar & 3 & screen & 4 \\
shoe-box & 1 & box & 1 & steamer & 3 & speaker & 6 \\
tray & 4 & milk-box & 4 & boxdrink & 4 & fan & 7 \\
kettle & 9 & mug & 13 & vagetable & 7 & seal & 6 \\
pen & 7 & rack & 1 & paymentsign & 4 & milk-tea & 6 \\
dustbin & 1 & shoe & 10 & can & 6 & roller & 3 \\
plant-pot & 5 & wooden\_box & 1 & electronicscale & 5 & fruit & 7 \\
dumbbell-rack & 4 & book & 2 & rubikscube & 3 & board & 5 \\
bookcase & 4 & microwave & 2 & displaystand & 5 & sauce-can & 5 \\
laptop & 11 & sand-clock & 3 & bread & 7 & skillet & 4 \\
oven & 4 & alarm-clock & 6 & breadbasket & 5 & soap & 4 \\
calculator & 6 & mouse & 3 & phone & 5 & block & 7 \\
microphone & 4 & stapler & 7 & phonestand & 7 & hydrating-oil & 4 \\
coaster & 1 & shampoo & 7 & remotecontrol & 7 & basket & 4 \\
hammer & 1 & bell & 2 & pillbottle & 5 & callbell & 6 \\
cup & 13 & candlestick & 5 & playingcards & 3 & tea-box & 6 \\
cup-with-liquid & 1 & dumbbell & 7 & smallshovel & 4 & coffee-box & 7 \\
tissue-box & 7 & teanet & 5 & brush & 4 & perfume & 4 \\
scanner & 5 & baguette & 2 & woodenmallet & 5 & keyboard & 4 \\
chips-tub & 4 & small-speaker & 3 & gong & 6 & whiteboard-eraser & 1 \\
pet-collar & 4 & switch & 8 & woodenblock & 5 & tooth-paste & 1 \\
table-tennis & 2 & toycar & 6 & waterer & 8 & mini-chalkboard & 1 \\
roll-paper & 4 & markpen & 6 & wineglass & 5 & plant & 1 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/datasets.tex <==
\begin{table*}[t]
\centering
\scriptsize
% \setlength{\tabcolsep}{2.2pt}
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lccccccccc}
\toprule
\textbf{Name} &
\textbf{Categories} &
\textbf{Tasks} &
\textbf{Trajectories} &
\textbf{Embodiments} &
\textbf{Spatial} &
\textbf{Long-Horizon} &
\textbf{Step-level} &
\textbf{Multi-} &
\textbf{Scene} \\
& & & & &
\textbf{Reasoning} &
\textbf{Tasks} &
\textbf{Evaluation} &
\textbf{Difficulty} &
\textbf{Diversity} \\
\midrule
% \multicolumn{10}{c}{Datasets} \\
% \midrule
BC-Z~\cite{jang2022bc}                         & 3   & 100+    & 26K          & 1  & \xmark & \xmark & \xmark & \xmark & \xmark \\
RT-1~\cite{Brohan-RSS-23}                      & 8   & 700+    & 130K         & 1  & \xmark & \cmark & \xmark & \xmark & \cmark \\
BridgeData V2~\cite{pmlr-v229-walke23a}        & --  & 13      & 60.1K        & 1  & \xmark & \xmark & \xmark & \xmark & \cmark \\
Open X-Embodiment~\cite{10611477}              & 527 & 160,266 & 1.4M         & 22 & \xmark & \xmark & \xmark & \xmark & \cmark \\
DROID~\cite{khazatsky2024droid}                & --  & 86      & 76K          & 1  & \xmark & \xmark & \xmark & \xmark & \cmark \\
\midrule
% \multicolumn{10}{c}{Benchmarks} \\
% \midrule
RLBench~\cite{james2019rlbenchrobotlearningbenchmark} 
                                                          & --  & 100     & --           & 1  & \xmark & \cmark & \xmark & \xmark & \xmark \\
CALVIN~\cite{9788026}                           & --  & 34      & N/A$^\dagger$& 1  & \xmark & \cmark & \cmark & \xmark & \cmark \\
LIBERO~\cite{liu2023libero}                     & 4   & 130     & 6.5K         & 1  & \xmark & \xmark & \xmark & \xmark & \cmark \\
ManiSkill2~\cite{gumaniskill2}                  & 4   & 20      & N/A$^\ddagger$ & 1  & \xmark & \xmark & \xmark & \xmark & \cmark \\
RoboCasa~\cite{Nasiriany-RSS-24}                & --  & 100     & $\sim$100K   & 1  & \xmark & \cmark & \xmark & \xmark & \cmark \\
SimplerEnv~\cite{pmlr-v270-li25c}                  & --  & 8       & --           & 2  & \xmark & \xmark & \xmark & \xmark & \cmark \\
MIKASA-Robo~\cite{cherepanov2026memory}         & 12  & 32      & 32K          & 1  & \xmark & \cmark & \xmark & \cmark & \xmark \\
RoboTwin 2.0~\cite{chen2026robotwin}            & --  & 50      & $\leq$137.5K & 5  & \xmark & \xmark & \xmark & \xmark & \cmark \\
LIBERO-Pro~\cite{zhou2025liberoprorobustfairevaluation} 
                                                          & 4   & 40      & --           & 1  & \xmark & \xmark & \xmark & \xmark & \cmark \\
RMBench~\cite{chen2026rmbenchmemorydependentroboticmanipulation} 
                                                          & 2   & 9       & 450          & 1  & \xmark & \cmark & \xmark & \xmark & \xmark \\
\midrule
\textbf{\texttt{RoboSPA} (Ours)}                            & 10  & 280     & 527K         & 5  & \cmark & \cmark & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
\caption{
Comparison of representative robotic manipulation datasets and benchmarks with \texttt{RoboSPA}. The upper and lower parts summarize datasets and benchmarks, respectively. $^\dagger$CALVIN reports approximately 24 hours of teleoperated demonstrations. 
$^\ddagger$ManiSkill2 reports over 4M demonstration frames. Spatial Reasoning indicates tasks with complex spatial attributes, while Long-Horizon Tasks indicates tasks with at least five steps.
}
\label{tab:dataset_comparison}
\end{table*}

==> tables/fail_modes.tex <==
\begin{table}[h]
\centering
\small
% \caption{Error types for spatial and long-horizon tasks.}
\caption{Definitions and descriptions of the error types.}
\label{tab:error_types}
\begin{tabular}{lp{8cm}}
\toprule
Error Type & Description \\
\midrule
Target Execution Error & The model selects the correct target but fails to execute the grasp or pick/place action properly. \\
No-Contact Grasp Error & The model attempts to grasp but fails to contact any object. \\
Target Grounding Error & The model selects the wrong object instead of the intended target or subtask object. \\
Temporal Ordering Error & Subtasks are executed in an incorrect order. \\
Redundant Repetition Error & The model repeats an already completed action instead of progressing to the next subgoal. \\
Manipulation Error & Low-level execution of a subtask fails (e.g., pick, pull, or move). \\
Memory Error & The model fails to retain relevant information from previous steps, affecting subtask completion. \\
\bottomrule
\end{tabular}
\end{table}

==> tables/main_table.tex <==


\begin{table*}[t]
\centering
\caption{
% \textbf{Performance comparison} of four baseline VLA models on our benchmark.
\textbf{Performance comparison} of four baseline VLA models on \texttt{RoboSPA} in terms of \textit{Success Rate} ($\mathcal{SR}$).
% Drop denotes the absolute performance decrease from L1 to L5.
Drop denotes the absolute performance decrease from the easiest (L1) to the hardest (L5) task.
\colorbox{blue!15}{Blue} shading highlights the best-performing model for each metric.}
\label{tab:main_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{Task}
& \multicolumn{3}{c}{RDT}
& \multicolumn{3}{c}{GO-1}
& \multicolumn{3}{c}{$\pi_{0.5}$}
& \multicolumn{3}{c}{X-VLA} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
& L1 & L5 & Drop
& L1 & L5 & Drop
& L1 & L5 & Drop
& L1 & L5 & Drop \\
\midrule

\multicolumn{13}{c}{Fine-Grained Spatial Reasoning} \\
\midrule
Geometric Attribute Cognition 
& 10.0 & 4.8 & 5.2 
& 27.8 & 11.5 & 16.3 
& 42.8 & 12.5 & 30.3 
& \cellcolor{blue!15}57.8 & \cellcolor{blue!15}25.3 & 32.5 \\
Spatial Distance Estimation 
& 15.2 & 9.4 & 5.8 
& 20.2 & 11.6 & 8.6 
& 35.0 & 23.4 & 11.6 
& \cellcolor{blue!15}41.4 & \cellcolor{blue!15}34.6 & 6.8 \\
Canonical Position Indexing 
& 15.0 & 8.6 & 6.4 
& 22.0 & 7.2 & 14.8 
& \cellcolor{blue!15}44.0 & \cellcolor{blue!15}23.6 & 20.4 
& 31.8 & 8.8 & 23.0 \\
Referential Relational Understanding 
& 4.4 & 4.4 & 0.0 
& 17.2 & 6.6 & 10.6 
& 33.2 & 9.8 & 23.4 
& \cellcolor{blue!15}40.4 & \cellcolor{blue!15}14.2 & 28.2 \\

Cross-View Reasoning 
& 3.0 & 3.4 & -0.4 
& 17.4 & 16.2 & 1.2 
& \cellcolor{blue!15}41.2 & \cellcolor{blue!15}37.6 & 3.6 
& 38.2 & 36.6 & 1.6 \\


\textit{Average} 
& 9.5 & 6.1 & 3.4 
& 20.9 & 10.6 & 10.3 
& 39.2 & 21.4 & 17.8 
& \cellcolor{blue!15}41.9 & \cellcolor{blue!15}23.9 & 18.0 \\


\midrule
\multicolumn{13}{c}{Long-Horizon Procedural Planning} \\
\midrule
Repetitive Procedure Following 
& 40.8 & 35.0 & 5.8 
& 31.8 & 23.8 & 8.0 
& \cellcolor{blue!15}80.3 & \cellcolor{blue!15}65.0 & 15.3 
& 34.8 & 22.5 & 12.3 \\
Order-Free Execution 
& 20.3 & 0.8 & 19.5 
& 41.1 & 5.6 & 35.5 
& 85.8 & 26.1 & 59.7 
& \cellcolor{blue!15}86.0 & \cellcolor{blue!15}43.6 & 42.4 \\
Order-Constrained Execution 
& 13.6 & 0.1 & 13.5 
& 41.9 & 3.1 & 38.8 
& \cellcolor{blue!15}77.4 & \cellcolor{blue!15}12.0 & 65.4 
& 70.0 & 7.7 & 62.3 \\
Composite Action Coordination 
& 27.5 & 2.4 & 25.1 
& 24.2 & 2.6 & 21.6 
& 58.6 & \cellcolor{blue!15}12.5 & 46.1 
& \cellcolor{blue!15}58.9 & 5.9 & 53.0 \\
Memory-Intensive Planning 
& 18.2 & \cellcolor{blue!15}0.0 & 18.2 
& 7.6 & \cellcolor{blue!15}0.0 & 7.6 
& \cellcolor{blue!15}54.0 & \cellcolor{blue!15}0.0 & 54.0 
& 44.6 & \cellcolor{blue!15}0.0 & 44.6 \\
\textit{Average} 
& 24.1 & 7.7 & 16.4 
& 29.3 & 7.0 & 22.3 
& \cellcolor{blue!15}71.2 & \cellcolor{blue!15}23.1 & 48.1 
& 58.8 & 15.9 & 42.9 \\

\midrule
\multicolumn{13}{c}{Overall Benchmark} \\
\midrule
\textit{Overall Average} 
& 16.8 & 6.9 & 9.9 
& 25.1 & 8.8 & 16.3 
& \cellcolor{blue!15}55.2 & \cellcolor{blue!15}22.3 & 32.9 
& 50.4 & 19.9 & 30.5 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/model_results_ONTA.tex <==

\begin{table}[H]
\centering
\caption{RDT per-task \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$) across difficulty levels (two-column format). Fine-grained spatial reasoning tasks only.}
\label{tab:appendix-rdt-onta}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & -94.0 & -48.5 & -29.3 & -17.5 & -18.8 & Pick Mixed Objects Canonical A & -33.5 & -15.2 & -8.6 & -11.4 & -3.6 \\
Pick Blocks Height & -44.0 & -18.5 & -6.7 & -6.3 & -5.6 & Pick Mixed Objects Canonical B & -21.5 & -12.8 & -8.6 & -5.8 & -4.7 \\
Pick Blocks Length & -88.0 & -48.5 & -32.0 & -20.0 & -16.4 & Pick Tea Box Referential & -86.0 & -47.0 & -26.7 & -12.8 & -9.1 \\
Pick Blocks Area & -94.0 & -48.5 & -32.0 & -18.8 & -16.4 & Pick Cans Referential & -96.0 & -48.5 & -24.0 & -14.0 & -5.8 \\
Pick Blocks Distance & -48.5 & -12.8 & -13.1 & -9.1 & -6.7 & Pick Soaps Referential & -84.0 & -32.0 & -21.3 & -14.0 & -4.6 \\
Pick Mugs Distance & -27.5 & -10.7 & -10.0 & -4.4 & -5.0 & Pick Mixed Objects Referential A & -96.0 & -47.0 & -24.0 & -11.6 & -8.0 \\
Pick Pill Bottles Distance & -12.5 & -13.3 & -7.5 & -4.4 & -1.5 & Pick Mixed Objects Referential B & -94.0 & -47.0 & -29.3 & -15.2 & -10.3 \\
Pick Mixed Objects Distance A & -27.5 & -12.0 & -7.5 & -12.8 & -5.0 & Pick Sauce Can Multi View & -45.5 & -26.7 & -28.0 & -29.3 & -24.0 \\
Pick Mixed Objects Distance B & -20.0 & -16.0 & -7.5 & -4.4 & -5.0 & Pick Seals Multi View & -45.5 & -26.7 & -26.7 & -28.0 & -28.0 \\
Pick Blocks Canonical & -45.5 & -14.0 & -9.7 & -11.4 & -3.6 & Pick Breads Multi View & -45.5 & -26.7 & -30.7 & -29.3 & -33.3 \\
Pick Cups Canonical & 2.5 & 1.6 & 9.7 & 6.6 & 14.9 & Pick Mixed Objects Multi View A & -48.5 & -26.7 & -30.7 & -29.3 & -28.0 \\
Pick Rubik Cubes Canonical & -39.5 & -12.8 & -7.4 & -4.6 & -1.5 & Pick Mixed Objects Multi View B & -42.5 & -32.0 & -28.0 & -29.3 & -30.7 \\
\bottomrule
\end{tabular}%
}
\end{table}

\vspace{0.75em}




\clearpage



\begin{table}[H]
\centering
\caption{GO-1 per-task \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$) across difficulty levels (two-column format). Fine-grained spatial reasoning tasks only.}
\label{tab:appendix-go1-onta}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & -34.0 & -30.5 & -17.3 & -12.5 & -9.2 & Pick Mixed Objects Canonical A & -18.5 & -5.6 & -7.4 & -5.8 & -4.7 \\
Pick Blocks Height & 42.0 & 43.0 & 33.3 & 33.8 & 18.4 & Pick Mixed Objects Canonical B & -15.5 & -2.0 & -6.3 & -8.0 & -5.8 \\
Pick Blocks Length & -94.0 & -33.5 & -13.3 & -16.3 & -14.0 & Pick Tea Box Referential & -58.0 & -24.5 & -9.3 & -9.2 & -4.6 \\
Pick Blocks Area & -92.0 & -45.5 & -30.7 & -25.0 & -20.0 & Pick Cans Referential & -68.0 & -32.0 & -28.0 & -3.2 & -3.5 \\
Pick Blocks Distance & -45.5 & -17.6 & -7.4 & -8.0 & -7.8 & Pick Soaps Referential & -76.0 & -38.0 & -28.0 & -16.4 & -9.1 \\
Pick Mugs Distance & -27.5 & -14.7 & -7.5 & -10.4 & -6.2 & Pick Mixed Objects Referential A & -60.0 & -23.0 & -16.0 & -2.0 & -2.4 \\
Pick Pill Bottles Distance & 4.0 & -22.7 & -6.3 & -2.0 & 13.7 & Pick Mixed Objects Referential B & -66.0 & -27.5 & -13.3 & -3.2 & -5.8 \\
Pick Mixed Objects Distance A & -11.0 & -8.0 & -5.0 & 2.8 & -2.7 & Pick Sauce Can Multi View & -8.0 & 10.7 & 8.0 & 5.3 & 2.7 \\
Pick Mixed Objects Distance B & -18.5 & -10.7 & -7.5 & -10.4 & -7.3 & Pick Seals Multi View & -23.0 & -13.3 & -14.7 & -17.3 & -18.7 \\
Pick Blocks Canonical & -26.0 & -6.8 & -5.1 & -5.8 & -1.5 & Pick Breads Multi View & -18.5 & -17.3 & -21.3 & 2.7 & -13.3 \\
Pick Cups Canonical & -14.0 & 0.4 & 0.6 & -3.5 & -1.5 & Pick Mixed Objects Multi View A & -26.0 & -22.7 & -28.0 & -9.3 & -9.3 \\
Pick Rubik Cubes Canonical & -11.0 & 0.4 & 1.7 & 2.1 & 7.3 & Pick Mixed Objects Multi View B & -44.0 & -28.0 & -17.3 & -17.3 & -20.0 \\
\bottomrule
\end{tabular}%
}
\end{table}





\vspace{0.75em}


\begin{table}[H]
\centering
\caption{$\pi_{0.5}$ per-task \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$) across difficulty levels (two-column format). Fine-grained spatial reasoning tasks only.}
\label{tab:appendix-pi05-onta}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & 16.0 & -9.5 & -6.7 & -3.8 & -4.4 & Pick Mixed Objects Canonical A & 2.5 & -2.0 & -2.9 & -0.1 & 2.9 \\
Pick Blocks Height & 34.0 & 31.0 & 30.7 & 12.5 & 8.8 & Pick Mixed Objects Canonical B & -2.0 & -2.0 & -2.9 & -1.2 & -1.5 \\
Pick Blocks Length & -56.0 & -42.5 & -18.7 & -20.0 & -16.4 & Pick Tea Box Referential & -34.0 & -3.5 & 8.0 & -5.6 & 4.4 \\
Pick Blocks Area & -52.0 & -30.5 & 0.0 & -10.0 & -8.0 & Pick Cans Referential & -46.0 & -18.5 & 4.0 & 0.4 & -3.5 \\
Pick Blocks Distance & -26.0 & -0.8 & 4.0 & -1.2 & 1.1 & Pick Soaps Referential & 6.0 & 16.0 & 17.3 & 2.8 & -1.2 \\
Pick Mugs Distance & 8.5 & 34.7 & 40.0 & 38.8 & 27.7 & Pick Mixed Objects Referential A & -34.0 & -24.5 & -17.3 & -5.6 & -3.5 \\
Pick Pill Bottles Distance & 19.0 & 14.7 & 13.8 & 19.6 & 21.8 & Pick Mixed Objects Referential B & -60.0 & -18.5 & -9.3 & 1.6 & -3.5 \\
Pick Mixed Objects Distance A & -0.5 & 16.0 & 8.8 & 14.8 & 10.2 & Pick Sauce Can Multi View & 20.5 & 30.7 & 24.0 & 22.7 & 22.7 \\
Pick Mixed Objects Distance B & 11.5 & 5.3 & 1.3 & 22.0 & -2.7 & Pick Seals Multi View & -2.0 & 8.0 & 8.0 & 8.0 & 6.7 \\
Pick Blocks Canonical & 11.5 & 6.4 & 1.7 & -1.2 & 2.9 & Pick Breads Multi View & 34.0 & 34.7 & 38.7 & 36.0 & 48.0 \\
Pick Cups Canonical & 41.5 & 24.4 & 31.4 & 33.6 & 40.0 & Pick Mixed Objects Multi View A & -0.5 & 2.7 & 2.7 & 10.7 & 9.3 \\
Pick Rubik Cubes Canonical & 26.5 & 22.0 & 23.4 & 28.0 & 38.9 & Pick Mixed Objects Multi View B & 7.0 & 5.3 & 6.7 & -4.0 & -2.7 \\
\bottomrule
\end{tabular}%
}
\end{table}



\vspace{0.75em}

\begin{table}[H]
\centering
\caption{X-VLA per-task \textit{Object-Normalized Target Accuracy} ($\mathcal{ONTA}$) across difficulty levels (two-column format). Fine-grained spatial reasoning tasks only.}
\label{tab:appendix-xvla-onta}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & -4.0 & -9.5 & -4.0 & 3.8 & -0.8 & Pick Mixed Objects Canonical A & -6.5 & -8.0 & 0.6 & -4.6 & -1.5 \\
Pick Blocks Height & 76.0 & 71.5 & 53.3 & 45.0 & 46.0 & Pick Mixed Objects Canonical B & -5.0 & -2.0 & 2.9 & 2.1 & -2.5 \\
Pick Blocks Length & -14.0 & -5.0 & -5.3 & 10.0 & -3.2 & Pick Tea Box Referential & -14.0 & 7.0 & 2.7 & 7.6 & 3.3 \\
Pick Blocks Area & 4.0 & -9.5 & 0.0 & 10.0 & -0.8 & Pick Cans Referential & -28.0 & -17.0 & -8.0 & 8.8 & 2.1 \\
Pick Blocks Distance & 8.5 & 32.8 & 23.4 & 20.1 & 25.6 & Pick Soaps Referential & -14.0 & -5.0 & 8.0 & -2.0 & 3.3 \\
Pick Mugs Distance & 16.0 & 22.7 & 6.3 & 14.8 & 10.2 & Pick Mixed Objects Referential A & -28.0 & -18.5 & 1.3 & -3.2 & 6.6 \\
Pick Pill Bottles Distance & 1.0 & 22.7 & 27.5 & 20.8 & 58.0 & Pick Mixed Objects Referential B & -12.0 & 1.0 & -2.7 & -0.8 & 2.1 \\
Pick Mixed Objects Distance A & 13.0 & 20.0 & 20.0 & 20.8 & 13.7 & Pick Sauce Can Multi View & 31.0 & 37.3 & 49.3 & 42.7 & 45.3 \\
Pick Mixed Objects Distance B & 22.0 & 20.0 & 13.8 & 24.4 & 14.8 & Pick Seals Multi View & -5.0 & 17.3 & 9.3 & 6.7 & 13.3 \\
Pick Blocks Canonical & 4.0 & 7.6 & -2.9 & -1.2 & -0.4 & Pick Breads Multi View & 5.5 & 16.0 & 10.7 & 21.3 & 12.0 \\
Pick Cups Canonical & 7.0 & 7.6 & 8.6 & 8.9 & 2.9 & Pick Mixed Objects Multi View A & 11.5 & 4.0 & 6.7 & 4.0 & -4.0 \\
Pick Rubik Cubes Canonical & -11.0 & 1.6 & 1.7 & -6.9 & 4.0 & Pick Mixed Objects Multi View B & -6.5 & 2.7 & 10.7 & 14.7 & 10.7 \\
\bottomrule
\end{tabular}%
}
\end{table}

\vspace{0.75em}





==> tables/model_results_PS.tex <==

% RDT step, generated from RDT.xlsx
% \begin{center}
% \captionsetup{type=table,hypcap=false}
% \caption{RDT per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
% \label{tab:appendix-rdt-step}
% \scriptsize
% \setlength{\tabcolsep}{2.6pt}
% \renewcommand{\arraystretch}{1.04}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrr@{\hspace{1.5em}}lrrrrr@{}}
\begin{table}[H]
\centering
\caption{RDT per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
\label{tab:appendix-rdt-step}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Press Stapler Repeat & 33.0 & 37.0 & 39.3 & 36.5 & 35.2 & Stack Blocks Color Order & 11.0 & 50.0 & 33.7 & 25.0 & 20.2 \\
Lift Pot Repeat & 76.0 & 75.5 & 75.7 & 72.0 & 80.0 & Stack Blocks Size Order & 9.0 & 0.0 & 33.7 & 25.3 & 20.4 \\
Lift Fan Repeat & 39.0 & 41.5 & 41.3 & 29.8 & 34.0 & Stack Blocks Length Order & 7.0 & 50.0 & 34.0 & 25.3 & 20.4 \\
Click Bell Repeat & 15.0 & 21.5 & 28.7 & 26.5 & 28.6 & Place Phone Press Stapler & 18.0 & 40.0 & 44.0 & 49.3 & 38.2 \\
Put Bottles Dustbin & 51.0 & 56.0 & 48.3 & 33.8 & 33.6 & Place Bottle Cup & 56.0 & 52.5 & 52.7 & 44.3 & 33.6 \\
Move Blocks Apart & 6.0 & 7.0 & 12.7 & 11.0 & 8.0 & Hang Mug Stack Blocks & 10.0 & 9.0 & 17.7 & 13.0 & 9.6 \\
Move Playing Cards Away & 8.0 & 13.0 & 8.0 & 9.0 & 10.6 & Place Object Scale Click & 39.0 & 41.5 & 41.3 & 29.8 & 34.0 \\
Place Bowls Plates & 48.0 & 37.5 & 39.0 & 32.3 & 20.6 & Place Burger Fries Click Bell & 33.0 & 23.5 & 17.7 & 15.3 & 11.4 \\
Separate Fries Bread & 24.0 & 26.0 & 33.0 & 28.0 & 35.4 & Click Can Place Items & 62.0 & 55.5 & 75.7 & 55.0 & 65.0 \\
Rank Blocks Height & 6.0 & 50.5 & 40.0 & 37.8 & 31.4 & Stamp Seals Press Stapler & 2.0 & 5.0 & 1.3 & 0.8 & 3.0 \\
Rank Blocks Color & 14.0 & 53.0 & 44.3 & 37.5 & 31.4 & Click Open Place & 0.0 & 16.5 & 10.0 & 22.8 & 17.2 \\
Rank Blocks Size & 5.0 & 50.0 & 38.3 & 33.8 & 28.0 & Observe Blocks Move Memory & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
Hit Blocks Hammer Order & 40.0 & 14.5 & 9.3 & 6.5 & 7.2 & Observe Objects Click Memory & 14.0 & 7.0 & 5.3 & 6.3 & 5.8 \\
Click Objects Order & 20.0 & 23.5 & 22.7 & 17.5 & 0.0 & Remember Color Cover & 47.0 & 23.5 & 15.0 & 5.5 & 6.0 \\
Stamp Seals Order & 3.0 & 3.0 & 5.7 & 6.3 & 6.6 & Remember Orientation Restore & 0.0 & 0.5 & 0.7 & 0.0 & 0.2 \\
Click Bell Clockwise Order & 5.0 & 50.0 & 38.3 & 33.8 & 28.0 & Press Stapler Memory & 30.0 & 7.0 & 4.0 & 3.3 & 5.8 \\
\bottomrule
\end{tabular}%
}
\end{table}
\vspace{0.75em}








% \clearpage

% PI05 step, generated from V2-pi05统计.xlsx
% \begin{center}
% \captionsetup{type=table,hypcap=false}
% \caption{$\pi_{0.5}$ per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
% \label{tab:appendix-pi05-step}
% \scriptsize
% \setlength{\tabcolsep}{2.6pt}
% \renewcommand{\arraystretch}{1.04}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrr@{\hspace{1.5em}}lrrrrr@{}}

\begin{table}[H]
\centering
\caption{GO-1 per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
\label{tab:appendix-go1-step}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Press Stapler Repeat & 27.0 & 25.5 & 14.7 & 8.3 & 8.8 & Stack Blocks Color Order & 54.0 & 56.0 & 36.7 & 25.8 & 20.0 \\
Lift Pot Repeat & 61.0 & 54.0 & 92.0 & 92.8 & 91.6 & Stack Blocks Size Order & 38.0 & 16.5 & 5.0 & 4.3 & 4.2 \\
Lift Fan Repeat & 23.0 & 22.5 & 24.7 & 26.5 & 21.2 & Stack Blocks Length Order & 30.0 & 12.0 & 10.3 & 4.3 & 3.0 \\
Click Bell Repeat & 16.0 & 19.0 & 8.7 & 9.3 & 6.3 & Place Phone Press Stapler & 48.0 & 33.0 & 34.3 & 30.0 & 28.8 \\
Put Bottles Dustbin & 59.0 & 84.5 & 68.0 & 60.3 & 48.4 & Place Bottle Cup & 16.0 & 16.5 & 50.3 & 68.5 & 57.0 \\
Move Blocks Apart & 21.0 & 21.5 & 12.0 & 8.3 & 6.6 & Hang Mug Stack Blocks & 8.0 & 23.3 & 18.5 & 18.3 & 13.1 \\
Move Playing Cards Away & 52.0 & 43.5 & 45.0 & 20.5 & 21.0 & Place Object Scale Click & 12.0 & 19.0 & 14.3 & 6.8 & 8.2 \\
Place Bowls Plates & 37.0 & 36.0 & 35.0 & 26.8 & 20.8 & Place Burger Fries Click Bell & 37.0 & 32.5 & 13.7 & 5.0 & 6.6 \\
Separate Fries Bread & 44.0 & 37.5 & 26.7 & 27.8 & 14.6 & Click Can Place Items & 77.0 & 45.5 & 53.3 & 51.0 & 55.4 \\
Rank Blocks Height & 34.0 & 51.5 & 39.3 & 36.0 & 30.0 & Stamp Seals Press Stapler & 24.0 & 23.0 & 8.3 & 5.3 & 5.2 \\
Rank Blocks Color & 41.0 & 57.0 & 44.7 & 36.5 & 30.6 & Click Open Place & 12.0 & 13.0 & 7.0 & 0.0 & 5.8 \\
Rank Blocks Size & 41.0 & 61.0 & 47.3 & 40.5 & 34.0 & Observe Blocks Move Memory & 3.0 & 3.0 & 1.3 & 11.0 & 11.6 \\
Hit Blocks Hammer Order & 36.0 & 29.0 & 24.3 & 27.5 & 27.0 & Observe Objects Click Memory & 19.0 & 6.5 & 8.3 & 5.8 & 5.2 \\
Click Objects Order & 62.0 & 42.0 & 30.3 & 24.3 & 3.0 & Remember Color Cover & 5.0 & 0.0 & 0.0 & 0.3 & 0.0 \\
Stamp Seals Order & 12.0 & 29.5 & 24.0 & 23.3 & 21.4 & Remember Orientation Restore & 2.0 & 6.0 & 5.7 & 6.5 & 5.4 \\
Click Bell Clockwise Order & 61.0 & 52.0 & 38.3 & 30.8 & 25.2 & Press Stapler Memory & 9.0 & 6.5 & 9.3 & 9.5 & 7.6 \\
\bottomrule
\end{tabular}%
}
\end{table}
\vspace{0.75em}

\begin{table}[H]
\centering
\caption{$\pi_{0.5}$ per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
\label{tab:appendix-pi05-step}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Press Stapler Repeat & 79.0 & 61.5 & 63.0 & 59.0 & 64.8 & Stack Blocks Color Order & 91.0 & 80.0 & 58.7 & 37.0 & 23.8 \\
Lift Pot Repeat & 60.0 & 64.5 & 77.0 & 71.8 & 74.8 & Stack Blocks Size Order & 89.0 & 75.0 & 49.3 & 36.3 & 25.0 \\
Lift Fan Repeat & 89.0 & 85.0 & 84.0 & 80.8 & 75.4 & Stack Blocks Length Order & 83.0 & 65.5 & 52.0 & 33.3 & 27.0 \\
Click Bell Repeat & 93.0 & 89.0 & 90.7 & 98.0 & 94.2 & Place Phone Press Stapler & 46.0 & 31.0 & 34.7 & 32.5 & 26.6 \\
Put Bottles Dustbin & 95.0 & 90.5 & 93.0 & 87.8 & 82.4 & Place Bottle Cup & 97.0 & 90.0 & 87.3 & 86.3 & 75.8 \\
Move Blocks Apart & 73.0 & 67.5 & 62.0 & 61.5 & 55.6 & Hang Mug Stack Blocks & 15.0 & 48.0 & 44.3 & 26.5 & 23.6 \\
Move Playing Cards Away & 81.0 & 78.5 & 77.3 & 81.5 & 77.8 & Place Object Scale Click & 19.0 & 50.5 & 56.0 & 22.8 & 30.2 \\
Place Bowls Plates & 94.0 & 91.5 & 78.0 & 69.5 & 50.4 & Place Burger Fries Click Bell & 87.0 & 90.0 & 78.0 & 61.8 & 72.0 \\
Separate Fries Bread & 92.0 & 88.5 & 83.0 & 86.8 & 74.4 & Click Can Place Items & 78.0 & 69.0 & 78.3 & 69.0 & 73.0 \\
Rank Blocks Height & 72.0 & 72.5 & 63.7 & 68.0 & 53.0 & Stamp Seals Press Stapler & 77.0 & 86.0 & 50.0 & 48.8 & 45.0 \\
Rank Blocks Color & 88.0 & 77.5 & 73.0 & 68.5 & 55.4 & Click Open Place & 50.0 & 48.5 & 55.0 & 30.8 & 37.4 \\
Rank Blocks Size & 91.0 & 84.0 & 69.7 & 57.5 & 47.8 & Observe Blocks Move Memory & 21.0 & 15.0 & 16.0 & 13.5 & 14.4 \\
Hit Blocks Hammer Order & 81.0 & 33.0 & 27.3 & 23.3 & 19.8 & Observe Objects Click Memory & 97.0 & 58.5 & 33.0 & 25.5 & 14.4 \\
Click Objects Order & 60.0 & 35.0 & 27.0 & 28.0 & 15.0 & Remember Color Cover & 100.0 & 50.5 & 20.3 & 12.0 & 7.0 \\
Stamp Seals Order & 40.0 & 50.5 & 43.0 & 43.6 & 46.6 & Remember Orientation Restore & 20.0 & 12.0 & 14.7 & 13.3 & 12.0 \\
Click Bell Clockwise Order & 98.0 & 96.5 & 52.7 & 40.8 & 38.6 & Press Stapler Memory & 32.0 & 10.0 & 9.7 & 8.8 & 9.4 \\
\bottomrule
\end{tabular}%
}
\end{table}
\vspace{0.75em}

% \clearpage

% GO-1 step, generated from go1.xlsx
% \begin{center}
% \captionsetup{type=table,hypcap=false}
% \caption{GO-1 per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
% \label{tab:appendix-go1-step}
% \scriptsize
% \setlength{\tabcolsep}{2.6pt}
% \renewcommand{\arraystretch}{1.04}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrr@{\hspace{1.5em}}lrrrrr@{}}


% \clearpage


% X-VLA step, generated from xvla.xlsx
% \begin{center}
% \captionsetup{type=table,hypcap=false}
% \caption{X-VLA per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
% \label{tab:appendix-xvla-step}
% \scriptsize
% \setlength{\tabcolsep}{2.6pt}
% \renewcommand{\arraystretch}{1.04}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrr@{\hspace{1.5em}}lrrrrr@{}}
\begin{table}[H]
\centering
\caption{X-VLA per-task step \textit{Progress Score} across difficulty levels. Step tables include long-horizon tasks only.}
\label{tab:appendix-xvla-step}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Press Stapler Repeat & 49.0 & 42.5 & 40.3 & 38.8 & 36.6 & Stack Blocks Color Order & 99.0 & 96.5 & 79.0 & 54.5 & 37.8 \\
Lift Pot Repeat & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & Stack Blocks Size Order & 78.0 & 93.5 & 55.0 & 29.3 & 22.2 \\
Lift Fan Repeat & 61.0 & 79.5 & 72.0 & 71.8 & 66.2 & Stack Blocks Length Order & 99.0 & 87.5 & 73.7 & 41.8 & 24.2 \\
Click Bell Repeat & 29.0 & 28.5 & 27.0 & 23.3 & 24.8 & Place Phone Press Stapler & 51.0 & 45.5 & 46.7 & 43.5 & 43.8 \\
Put Bottles Dustbin & 79.0 & 80.0 & 78.3 & 71.0 & 74.0 & Place Bottle Cup & 98.0 & 71.0 & 61.3 & 49.0 & 40.0 \\
Move Blocks Apart & 86.0 & 80.5 & 89.7 & 65.0 & 71.2 & Hang Mug Stack Blocks & 23.0 & 51.0 & 51.7 & 41.3 & 31.4 \\
Move Playing Cards Away & 97.0 & 98.0 & 95.7 & 93.6 & 93.6 & Place Object Scale Click & 57.0 & 35.0 & 30.3 & 27.3 & 20.0 \\
Place Bowls Plates & 67.0 & 62.5 & 52.7 & 39.3 & 30.4 & Place Burger Fries Click Bell & 98.0 & 78.5 & 55.7 & 57.3 & 49.8 \\
Separate Fries Bread & 78.0 & 92.5 & 87.3 & 89.5 & 82.2 & Click Can Place Items & 54.0 & 64.5 & 67.7 & 69.3 & 64.2 \\
Rank Blocks Height & 91.0 & 97.5 & 93.3 & 91.0 & 83.0 & Stamp Seals Press Stapler & 75.0 & 89.0 & 61.0 & 49.3 & 42.8 \\
Rank Blocks Color & 93.0 & 96.5 & 95.0 & 92.5 & 90.0 & Click Open Place & 15.0 & 19.5 & 18.0 & 24.8 & 28.8 \\
Rank Blocks Size & 97.0 & 94.5 & 83.3 & 71.0 & 67.0 & Observe Blocks Move Memory & 46.0 & 29.5 & 27.7 & 27.3 & 19.4 \\
Hit Blocks Hammer Order & 84.0 & 57.5 & 46.7 & 40.5 & 30.8 & Observe Objects Click Memory & 18.0 & 4.5 & 5.0 & 2.8 & 2.6 \\
Click Objects Order & 39.0 & 20.0 & 10.3 & 6.5 & 0.0 & Remember Color Cover & 100.0 & 50.0 & 18.3 & 6.5 & 4.0 \\
Stamp Seals Order & 34.0 & 77.0 & 78.3 & 78.3 & 53.2 & Remember Orientation Restore & 18.0 & 19.5 & 7.0 & 6.3 & 5.6 \\
Click Bell Clockwise Order & 57.0 & 26.0 & 14.7 & 9.8 & 7.2 & Press Stapler Memory & 41.0 & 6.5 & 3.0 & 4.3 & 4.8 \\
\bottomrule
\end{tabular}%
}
\end{table}
\vspace{0.75em}



==> tables/model_results_SR.tex <==

\begin{table}[H]
\centering
\caption{RDT per-task \textit{Success Rate} across difficulty levels (two-column format).}
\label{tab:appendix-rdt-success}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & 3 & 1 & 3 & 6 & 1 & Put Bottles Dustbin & 51 & 37 & 22 & 8 & 2 \\
Pick Blocks Height & 28 & 21 & 20 & 15 & 12 & Move Blocks Apart & 6 & 2 & 1 & 0 & 0 \\
Pick Blocks Length & 6 & 1 & 1 & 4 & 3 & Move Playing Cards Away & 8 & 5 & 0 & 0 & 0 \\
Pick Blocks Area & 3 & 1 & 1 & 5 & 3 & Place Bowls Plates & 48 & 15 & 12 & 6 & 2 \\
Pick Blocks Distance & 1 & 6 & 1 & 3 & 4 & Separate Fries Bread & 24 & 9 & 6 & 1 & 2 \\
Pick Mugs Distance & 15 & 17 & 12 & 13 & 10 & Rank Blocks Height & 6 & 1 & 0 & 1 & 0 \\
Pick Pill Bottles Distance & 25 & 15 & 14 & 13 & 13 & Rank Blocks Color & 14 & 6 & 1 & 0 & 0 \\
Pick Mixed Objects Distance A & 15 & 16 & 14 & 6 & 10 & Rank Blocks Size & 5 & 0 & 0 & 0 & 0 \\
Pick Mixed Objects Distance B & 20 & 13 & 14 & 13 & 10 & Hit Blocks Hammer Order & 40 & 4 & 0 & 0 & 0 \\
Pick Blocks Canonical & 3 & 5 & 4 & 1 & 5 & Click Objects Order & 20 & 0 & 0 & 0 & 0 \\
Pick Cups Canonical & 35 & 18 & 21 & 17 & 22 & Stamp Seals Order & 3 & 0 & 1 & 1 & 1 \\
Pick Rubik Cubes Canonical & 7 & 6 & 6 & 7 & 7 & Click Bell Clockwise Order & 5 & 0 & 0 & 0 & 0 \\
Pick Mixed Objects Canonical A & 11 & 4 & 5 & 1 & 5 & Stack Blocks Color Order & 11 & 0 & 0 & 0 & 0 \\
Pick Mixed Objects Canonical B & 19 & 6 & 5 & 6 & 4 & Stack Blocks Size Order & 9 & 0 & 0 & 0 & 0 \\
Pick Tea Box Referential & 7 & 2 & 5 & 6 & 3 & Stack Blocks Length Order & 7 & 0 & 0 & 0 & 0 \\
Pick Cans Referential & 2 & 1 & 7 & 5 & 6 & Place Phone Press Stapler & 18 & 6 & 1 & 0 & 0 \\
Pick Soaps Referential & 8 & 12 & 9 & 5 & 7 & Place Bottle Cup & 56 & 29 & 26 & 6 & 0 \\
Pick Mixed Objects Referential A & 2 & 2 & 7 & 7 & 4 & Hang Mug Stack Blocks & 10 & 0 & 0 & 0 & 0 \\
Pick Mixed Objects Referential B & 3 & 2 & 3 & 4 & 2 & Place Object Scale Click & 39 & 33 & 26 & 9 & 17 \\
Pick Sauce Can Multi View & 3 & 5 & 4 & 3 & 7 & Place Burger Fries Click Bell & 33 & 20 & 4 & 0 & 0 \\
Pick Seals Multi View & 3 & 5 & 5 & 4 & 4 & Click Can Place Items & 62 & 24 & 34 & 0 & 2 \\
Pick Breads Multi View & 3 & 5 & 2 & 3 & 0 & Stamp Seals Press Stapler & 2 & 3 & 0 & 0 & 0 \\
Pick Mixed Objects Multi View A & 1 & 5 & 2 & 3 & 4 & Click Open Place & 0 & 1 & 2 & 0 & 0 \\
Pick Mixed Objects Multi View B & 5 & 1 & 4 & 3 & 2 & Observe Blocks Move Memory & 0 & 0 & 0 & 0 & 0 \\
Press Stapler Repeat & 33 & 37 & 37 & 34 & 32 & Observe Objects Click Memory & 14 & 0 & 0 & 0 & 0 \\
Lift Pot Repeat & 76 & 68 & 63 & 56 & 68 & Remember Color Cover & 47 & 14 & 6 & 0 & 0 \\
Lift Fan Repeat & 39 & 33 & 26 & 9 & 17 & Remember Orientation Restore & 0 & 0 & 0 & 0 & 0 \\
Click Bell Repeat & 15 & 17 & 22 & 22 & 23 & Press Stapler Memory & 30 & 3 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}%
}
\end{table}


\clearpage
\begin{table}[H]
\centering
\caption{GO-1 per-task \textit{Success Rate} across difficulty levels (two-column format).}
\label{tab:appendix-go1-success}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & 33 & 13 & 12 & 10 & 9 & Put Bottles Dustbin & 59 & 77 & 42 & 33 & 11 \\
Pick Blocks Height & 71 & 62 & 50 & 47 & 32 & Move Blocks Apart & 21 & 10 & 3 & 1 & 0 \\
Pick Blocks Length & 3 & 11 & 15 & 7 & 5 & Move Playing Cards Away & 52 & 39 & 33 & 13 & 17 \\
Pick Blocks Area & 4 & 3 & 2 & 0 & 0 & Place Bowls Plates & 37 & 23 & 21 & 13 & 5 \\
Pick Blocks Distance & 3 & 2 & 6 & 4 & 3 & Separate Fries Bread & 44 & 32 & 19 & 21 & 7 \\
Pick Mugs Distance & 15 & 14 & 14 & 8 & 9 & Rank Blocks Height & 34 & 3 & 0 & 0 & 0 \\
Pick Pill Bottles Distance & 36 & 8 & 15 & 15 & 26 & Rank Blocks Color & 41 & 14 & 8 & 5 & 2 \\
Pick Mixed Objects Distance A & 26 & 19 & 16 & 19 & 12 & Rank Blocks Size & 41 & 22 & 13 & 9 & 3 \\
Pick Mixed Objects Distance B & 21 & 17 & 14 & 8 & 8 & Hit Blocks Hammer Order & 36 & 11 & 3 & 3 & 1 \\
Pick Blocks Canonical & 16 & 11 & 8 & 6 & 7 & Click Objects Order & 62 & 11 & 6 & 4 & 3 \\
Pick Cups Canonical & 24 & 17 & 13 & 8 & 7 & Stamp Seals Order & 12 & 15 & 10 & 9 & 6 \\
Pick Rubik Cubes Canonical & 26 & 17 & 14 & 13 & 15 & Click Bell Clockwise Order & 61 & 48 & 34 & 21 & 12 \\
Pick Mixed Objects Canonical A & 21 & 12 & 6 & 6 & 4 & Stack Blocks Color Order & 54 & 12 & 3 & 1 & 0 \\
Pick Mixed Objects Canonical B & 23 & 15 & 7 & 4 & 3 & Stack Blocks Size Order & 38 & 11 & 1 & 0 & 0 \\
Pick Tea Box Referential & 21 & 17 & 18 & 9 & 7 & Stack Blocks Length Order & 30 & 7 & 5 & 0 & 0 \\
Pick Cans Referential & 16 & 12 & 4 & 14 & 8 & Place Phone Press Stapler & 48 & 14 & 14 & 5 & 1 \\
Pick Soaps Referential & 12 & 8 & 4 & 3 & 3 & Place Bottle Cup & 16 & 12 & 34 & 23 & 4 \\
Pick Mixed Objects Referential A & 20 & 18 & 13 & 15 & 9 & Hang Mug Stack Blocks & 8 & 2 & 0 & 0 & 0 \\
Pick Mixed Objects Referential B & 17 & 15 & 15 & 14 & 6 & Place Object Scale Click & 12 & 14 & 10 & 2 & 3 \\
Pick Sauce Can Multi View & 28 & 33 & 31 & 29 & 27 & Place Burger Fries Click Bell & 37 & 29 & 11 & 3 & 5 \\
Pick Seals Multi View & 18 & 15 & 14 & 12 & 11 & Click Can Place Items & 77 & 11 & 14 & 5 & 3 \\
Pick Breads Multi View & 21 & 12 & 9 & 27 & 15 & Stamp Seals Press Stapler & 24 & 17 & 2 & 0 & 0 \\
Pick Mixed Objects Multi View A & 16 & 8 & 4 & 18 & 18 & Click Open Place & 12 & 13 & 7 & 0 & 2 \\
Pick Mixed Objects Multi View B & 4 & 4 & 12 & 12 & 10 & Observe Blocks Move Memory & 3 & 0 & 0 & 0 & 0 \\
Press Stapler Repeat & 27 & 21 & 12 & 8 & 7 & Observe Objects Click Memory & 19 & 1 & 0 & 0 & 0 \\
Lift Pot Repeat & 61 & 53 & 83 & 84 & 77 & Remember Color Cover & 5 & 0 & 0 & 0 & 0 \\
Lift Fan Repeat & 23 & 17 & 17 & 21 & 11 & Remember Orientation Restore & 2 & 0 & 0 & 0 & 0 \\
Click Bell Repeat & 16 & 12 & 3 & 1 & 0 & Press Stapler Memory & 9 & 2 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}%
}
\end{table}


\vspace{0.75em}

\begin{table}[H]
\centering
\caption{$\pi_{0.5}$ per-task \textit{Success Rate} across difficulty levels (two-column format).}
\label{tab:appendix-pi05-success}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & 58 & 27 & 20 & 17 & 13 & Put Bottles Dustbin & 95 & 85 & 81 & 74 & 61 \\
Pick Blocks Height & 67 & 54 & 48 & 30 & 24 & Move Blocks Apart & 73 & 51 & 24 & 35 & 18 \\
Pick Blocks Length & 22 & 5 & 11 & 4 & 3 & Move Playing Cards Away & 81 & 64 & 54 & 52 & 47 \\
Pick Blocks Area & 24 & 13 & 25 & 12 & 10 & Place Bowls Plates & 94 & 85 & 61 & 52 & 22 \\
Pick Blocks Distance & 16 & 16 & 16 & 10 & 11 & Separate Fries Bread & 92 & 84 & 58 & 59 & 36 \\
Pick Mugs Distance & 39 & 51 & 52 & 49 & 38 & Rank Blocks Height & 72 & 45 & 19 & 24 & 6 \\
Pick Pill Bottles Distance & 46 & 36 & 31 & 33 & 33 & Rank Blocks Color & 88 & 50 & 46 & 36 & 11 \\
Pick Mixed Objects Distance A & 33 & 37 & 27 & 29 & 23 & Rank Blocks Size & 91 & 66 & 37 & 15 & 8 \\
Pick Mixed Objects Distance B & 41 & 29 & 21 & 22 & 12 & Hit Blocks Hammer Order & 81 & 30 & 14 & 7 & 3 \\
Pick Blocks Canonical & 41 & 22 & 14 & 10 & 11 & Click Objects Order & 60 & 29 & 16 & 13 & 15 \\
Pick Cups Canonical & 61 & 37 & 40 & 41 & 45 & Stamp Seals Order & 40 & 40 & 30 & 36 & 35 \\
Pick Rubik Cubes Canonical & 51 & 35 & 33 & 36 & 44 & Click Bell Clockwise Order & 98 & 95 & 45 & 31 & 28 \\
Pick Mixed Objects Canonical A & 35 & 15 & 10 & 11 & 11 & Stack Blocks Color Order & 91 & 58 & 25 & 5 & 1 \\
Pick Mixed Objects Canonical B & 32 & 15 & 10 & 10 & 7 & Stack Blocks Size Order & 89 & 43 & 4 & 3 & 0 \\
Pick Tea Box Referential & 33 & 31 & 31 & 12 & 15 & Stack Blocks Length Order & 83 & 27 & 18 & 3 & 2 \\
Pick Cans Referential & 27 & 21 & 28 & 17 & 8 & Place Phone Press Stapler & 46 & 14 & 17 & 12 & 1 \\
Pick Soaps Referential & 53 & 44 & 38 & 19 & 10 & Place Bottle Cup & 97 & 79 & 69 & 67 & 30 \\
Pick Mixed Objects Referential A & 33 & 17 & 12 & 12 & 8 & Hang Mug Stack Blocks & 15 & 8 & 3 & 0 & 0 \\
Pick Mixed Objects Referential B & 20 & 21 & 18 & 18 & 8 & Place Object Scale Click & 19 & 36 & 56 & 6 & 5 \\
Pick Sauce Can Multi View & 47 & 48 & 43 & 42 & 42 & Place Burger Fries Click Bell & 87 & 89 & 57 & 14 & 34 \\
Pick Seals Multi View & 32 & 31 & 31 & 31 & 30 & Click Can Place Items & 78 & 46 & 47 & 14 & 18 \\
Pick Breads Multi View & 56 & 51 & 54 & 52 & 61 & Stamp Seals Press Stapler & 77 & 82 & 8 & 7 & 1 \\
Pick Mixed Objects Multi View A & 33 & 27 & 27 & 33 & 32 & Click Open Place & 50 & 22 & 37 & 5 & 11 \\
Pick Mixed Objects Multi View B & 38 & 29 & 30 & 22 & 23 & Observe Blocks Move Memory & 21 & 0 & 0 & 0 & 0 \\
Press Stapler Repeat & 79 & 41 & 42 & 36 & 45 & Observe Objects Click Memory & 97 & 35 & 3 & 0 & 0 \\
Lift Pot Repeat & 60 & 43 & 63 & 54 & 63 & Remember Color Cover & 100 & 48 & 11 & 2 & 0 \\
Lift Fan Repeat & 89 & 80 & 73 & 71 & 62 & Remember Orientation Restore & 20 & 0 & 1 & 0 & 0 \\
Click Bell Repeat & 93 & 84 & 87 & 95 & 90 & Press Stapler Memory & 32 & 3 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}%
}
\end{table}



\vspace{0.75em}



\begin{table}[H]
\centering
\caption{X-VLA per-task \textit{Success Rate} across difficulty levels (two-column format).}
\label{tab:appendix-xvla-success}
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrr@{\hspace{1.2em}}lrrrrr@{}}
\toprule
Task & L1 & L2 & L3 & L4 & L5 & Task & L1 & L2 & L3 & L4 & L5 \\
\midrule
Pick Blocks Size & 48 & 27 & 22 & 23 & 16 & Put Bottles Dustbin & 79 & 64 & 55 & 31 & 28 \\
Pick Blocks Height & 88 & 81 & 65 & 56 & 55 & Move Blocks Apart & 86 & 74 & 81 & 17 & 31 \\
Pick Blocks Length & 43 & 30 & 21 & 28 & 14 & Move Playing Cards Away & 97 & 96 & 92 & 87 & 83 \\
Pick Blocks Area & 52 & 27 & 25 & 28 & 16 & Place Bowls Plates & 67 & 44 & 29 & 15 & 8 \\
Pick Blocks Distance & 39 & 44 & 33 & 29 & 33 & Separate Fries Bread & 78 & 87 & 71 & 79 & 66 \\
Pick Mugs Distance & 44 & 42 & 25 & 29 & 23 & Rank Blocks Height & 91 & 95 & 84 & 72 & 46 \\
Pick Pill Bottles Distance & 34 & 42 & 42 & 34 & 64 & Rank Blocks Color & 93 & 92 & 91 & 82 & 63 \\
Pick Mixed Objects Distance A & 42 & 40 & 36 & 34 & 26 & Rank Blocks Size & 97 & 88 & 65 & 32 & 24 \\
Pick Mixed Objects Distance B & 48 & 40 & 31 & 37 & 27 & Hit Blocks Hammer Order & 84 & 36 & 16 & 7 & 4 \\
Pick Blocks Canonical & 36 & 23 & 10 & 10 & 8 & Click Objects Order & 39 & 6 & 0 & 0 & 0 \\
Pick Cups Canonical & 38 & 23 & 20 & 19 & 11 & Stamp Seals Order & 34 & 71 & 65 & 65 & 31 \\
Pick Rubik Cubes Canonical & 26 & 18 & 14 & 5 & 12 & Click Bell Clockwise Order & 57 & 15 & 1 & 0 & 0 \\
Pick Mixed Objects Canonical A & 29 & 10 & 13 & 7 & 7 & Stack Blocks Color Order & 99 & 93 & 67 & 33 & 18 \\
Pick Mixed Objects Canonical B & 30 & 15 & 15 & 13 & 6 & Stack Blocks Size Order & 78 & 87 & 29 & 2 & 1 \\
Pick Tea Box Referential & 43 & 38 & 27 & 23 & 14 & Stack Blocks Length Order & 99 & 74 & 59 & 14 & 0 \\
Pick Cans Referential & 36 & 22 & 19 & 24 & 13 & Place Phone Press Stapler & 51 & 28 & 25 & 22 & 7 \\
Pick Soaps Referential & 43 & 30 & 31 & 15 & 14 & Place Bottle Cup & 98 & 44 & 19 & 16 & 6 \\
Pick Mixed Objects Referential A & 36 & 21 & 26 & 14 & 17 & Hang Mug Stack Blocks & 23 & 5 & 3 & 2 & 0 \\
Pick Mixed Objects Referential B & 44 & 34 & 23 & 16 & 13 & Place Object Scale Click & 57 & 22 & 19 & 5 & 2 \\
Pick Sauce Can Multi View & 54 & 53 & 62 & 57 & 59 & Place Burger Fries Click Bell & 98 & 59 & 18 & 12 & 4 \\
Pick Seals Multi View & 30 & 38 & 32 & 30 & 35 & Click Can Place Items & 54 & 41 & 37 & 34 & 24 \\
Pick Breads Multi View & 37 & 37 & 33 & 41 & 34 & Stamp Seals Press Stapler & 75 & 86 & 4 & 2 & 1 \\
Pick Mixed Objects Multi View A & 41 & 28 & 30 & 28 & 22 & Click Open Place & 3 & 2 & 0 & 0 & 0 \\
Pick Mixed Objects Multi View B & 29 & 27 & 33 & 36 & 33 & Observe Blocks Move Memory & 46 & 11 & 5 & 3 & 0 \\
Press Stapler Repeat & 49 & 35 & 30 & 29 & 27 & Observe Objects Click Memory & 18 & 0 & 0 & 0 & 0 \\
Lift Pot Repeat & 0 & 0 & 0 & 0 & 0 & Remember Color Cover & 100 & 48 & 8 & 0 & 0 \\
Lift Fan Repeat & 61 & 70 & 59 & 51 & 43 & Remember Orientation Restore & 18 & 6 & 0 & 0 & 0 \\
Click Bell Repeat & 29 & 24 & 20 & 19 & 20 & Press Stapler Memory & 41 & 1 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}%
}
\end{table}
\vspace{0.75em}


==> tables/tasks.tex <==




% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{19pt} % 默认约6pt，这里增大列间距
% \begin{tabular}{lccc}
% \toprule
% \textbf{Task Name} & \textbf{Success Rate} & \textbf{Avg Step Success Ratio} & \textbf{Avg Video Time} \\
% \midrule
% task\_1 &  &  &  \\
% task\_2 &  &  &  \\
% task\_3 &  &  &  \\
% task\_4 &  &  &  \\
% task\_5 &  &  &  \\
% % 可以按需继续添加
% \bottomrule
% \end{tabular}
% \caption{Performance metrics across different tasks.}
% \label{tab:task_metrics}
% \end{table}


% 两列版本
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{7.5pt} % 适当调整列间距，更美观
\begin{tabular}{lccc|lccc}
\toprule
\textbf{Task} & \textbf{Success Rate} & \textbf{Avg SSR} & \textbf{Avg VT} 
& \textbf{Task} & \textbf{Success Rate} & \textbf{Avg SSR} & \textbf{Avg VT} \\
\midrule
task\_1 &  &  &  & task\_6 &  &  &  \\
task\_2 &  &  &  & task\_7 &  &  &  \\
task\_3 &  &  &  & task\_8 &  &  &  \\
task\_4 &  &  &  & task\_9 &  &  &  \\
task\_5 &  &  &  & task\_10 &  &  &  \\
\bottomrule
\end{tabular}
\caption{Performance metrics across different tasks.}
\label{tab:task_metrics}
\end{table}

==> tables/v1.tex <==
\begin{table}[H]
\centering
\caption{Performance on basic spatial task variants. These tasks show relatively high success rates across difficulty levels, motivating more fine-grained spatial reasoning evaluation.}
\label{tab:basic_spatial_tasks}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Task} & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{L5} \\
\midrule
Color-based Target Selection & 80.6 & 77.8 & 79.8 & 71.2 & 74.0 \\
Absolute Position & 67.8 & 69.4 & 74.8 & 72.2 & 72.4 \\
Simple Ordinal Indexing & 87.0 & 86.8 & 83.8 & 87.0 & 84.8 \\
\bottomrule
\end{tabular}
\end{table}
